Mirror Descent Policy Optimization

Mirror descent (MD), a well-known first-order method in constrained convex optimization, has recently been shown as an important tool to analyze trust-region algorithms in reinforcement learning (RL). However, there remains a considerable gap between such theoretically analyzed algorithms and the ones used in practice. Inspired by this, we propose an efficient RL algorithm, called {\em mirror descent policy optimization} (MDPO). MDPO iteratively updates the policy by {\em approximately} solving a trust-region problem, whose objective function consists of two terms: a linearization of the standard RL objective and a proximity term that restricts two consecutive policies to be close to each other. Each update performs this approximation by taking multiple gradient steps on this objective function. We derive {\em on-policy} and {\em off-policy} variants of MDPO, while emphasizing important design choices motivated by the existing theory of MD in RL. We highlight the connections between on-policy MDPO and two popular trust-region RL algorithms: TRPO and PPO, and show that explicitly enforcing the trust-region constraint is in fact {\em not} a necessity for high performance gains in TRPO. We then show how the popular soft actor-critic (SAC) algorithm can be derived by slight modifications of off-policy MDPO. Overall, MDPO is derived from the MD principles, offers a unified approach to viewing a number of popular RL algorithms, and performs better than or on-par with TRPO, PPO, and SAC in a number of continuous control tasks. Code is available at \url{https://github.com/manantomar/Mirror-Descent-Policy-Optimization}.

==> Sections/Abstract.tex <==
\vspace{-0.25in}
\begin{abstract}
\vspace{-0.05in}
%We propose a deep reinforcement learning (RL) algorithm inspired by mirror descent (MD), a well-known first-order trust-region method in constrained convex optimization. Our algorithm, called {\em Mirror Descent Policy Optimization} (MDPO), is based on the idea of iteratively solving a trust-region problem that minimizes a sum of two terms: a linearization of the standard RL objective function and a proximity term that restricts two consecutive updates to be close to each other. We derive on-policy and off-policy variants of {\small MDPO} and empirically evaluate their performance on a range of continuous control tasks, while emphasizing important implementation details motivated by the existing theory of MD in RL. We highlight the connections between on-policy {\small MDPO} and two popular trust-region RL algorithms: {\small TRPO} and {\small PPO}, and show that a hard constraint on the policy update is in fact not a necessity for high performance gains. We then highlight the connection between off-policy {\small MDPO} and Soft Actor Critic, a popular off-policy method based on entropy regularization. Overall, {\small MDPO} is derived from the MD principles, offers a unified approach to viewing a number of popular RL algorithms, and achieves strong performance across a variety of tasks. 

%Mirror Descent (MD) has recently been used as an important tool for providing theoretical guarantees in the policy optimization literature in RL \cite{geist2019theory, neu2017unified, shani2019adaptive}. In this paper, we take a big step towards applying such analysis tools in developing practical and efficient deep RL algorithms with strong theoretical motivation. To this end, we develop {\em Mirror Descent Policy Optimization} (MDPO), a method based on the idea of iteratively solving a trust-region problem that optimizes a sum of two terms: a linearization of the standard RL objective function and a proximity term that restricts two consecutive updates to be close to each other. However, when the policy is parameterized by a function class, a closed form solution does not usually exist. We test a natural solution to this problem: solving the trust region problem with gradient descent. We derive on-policy and off-policy variants of {\small MDPO}, while emphasizing important design choices motivated by the existing theory of MD in RL. Interestingly, we highlight the connections between on-policy {\small MDPO} and two popular trust-region RL algorithms: {\small TRPO} and {\small PPO}, and show that a hard constraint on the policy update is in fact not a necessity for high performance gains. We then highlight how a special case of off-policy {\small MDPO} leads to Soft Actor Critic, a popular off-policy method based on entropy regularization. Overall, {\small MDPO} is derived from the MD principles, offers a unified approach to viewing a number of popular RL algorithms, and outperforms the state-of-the-art in on-policy while achieving similar performance in the off-policy cases.

Mirror descent (MD), a well-known first-order method in constrained convex optimization, has recently been shown as an important tool to analyze trust-region algorithms in reinforcement learning (RL). However, there remains a considerable gap between such theoretically analyzed algorithms and the ones used in practice. Inspired by this, we propose an efficient RL algorithm, called {\em mirror descent policy optimization} (MDPO). MDPO iteratively updates the policy by {\em approximately} solving a trust-region problem, whose objective function consists of two terms: a linearization of the standard RL objective and a proximity term that restricts two consecutive policies to be close to each other. Each update performs this approximation by taking multiple gradient steps on this objective function. We derive {\em on-policy} and {\em off-policy} variants of MDPO, while emphasizing important design choices motivated by the existing theory of MD in RL. We highlight the connections between on-policy MDPO and two popular trust-region RL algorithms: TRPO and PPO, and show that explicitly enforcing the trust-region constraint is in fact {\em not} a necessity for high performance gains in TRPO. We then show how the popular soft actor-critic (SAC) algorithm can be derived by slight modifications of off-policy MDPO. Overall, MDPO is derived from the MD principles, offers a unified approach to viewing a number of popular RL algorithms, and performs better than or on-par with TRPO, PPO, and SAC in a number of continuous control tasks.


% In on-policy MDPO, we generate the next policy by performing multiple gradient updates of the sum, while in off-policy MDPO, we first lift the policy to the simplex, to remove the parametrization constraint, and then approximately solve the projection by gradient updates in the parameter space. We establish the connection between on-policy MDPO and two popular trust region RL algorithms: TRPO and PPO, and conduct a comprehensive empirical comparison of these algorithms. We then extend off-policy MDPO to incorporate entropy regularization, and study its relationship with the Soft Actor-Critic (SAC) algorithm, followed by empirical comparisons. Our experimental results on MuJoCo benchmarks show that both on-policy and off-policy MDPO outperform or are on par with TRPO, PPO, and SAC. 

%However, when using non-linear function approximations, solving the trust-region problem does not have a close form. In this work, we test a simple heuristic solution to this problem: \emph{solve the trust-region problem with gradient descent}. We test this approach in both on-policy and off-policy cases. Furthermore, we establish the connection between on-policy MDPO and two popular trust region RL algorithms: TRPO and PPO, and conduct a comprehensive empirical comparison of these algorithms. 
% We then extend off-policy MDPO to incorporate entropy regularization, and study its relationship with the Soft Actor-Critic (SAC) algorithm, followed by empirical comparisons. Our experimental results on MuJoCo benchmarks show that both on-policy and off-policy MDPO outperform or are on par with TRPO, PPO, and SAC \lior{Do you think we should say on par?}. 

%We develop two versions of MDPO, resulting in On-policy and Off-policy variants. We establish connections between On-policy MDPO and Trust Region Policy Optimization methods (i.e. TRPO and PPO), which is followed by an empirical comparison. We then extend Off Policy MDPO to incorporate entropy regularization and show similarities to Soft Actor Critic (SAC). A similar empirical comparison follows and finally, we show that MDPO outperforms or is on-par with the mentioned RL methods when evaluated on the Mujoco domain. In addition, MDPO remains closely attached to the supporting theory and efficient in ease of implementation.  


% Trust region methods are a popular class of algorithms to solve the reinforcement learning problem. These methods iteratively solve constraint optimization problem which keeps consecutive policies close to one another. Recently,  minimize a linearized objective function and a proximity term which restricts two consecutive updates to be close to each other

%that use mirror descent . We call our algorithms mirror descent policy optimization (MDPO)

%In the mirror descent approach to policy optimization, we iteratively minimize a sum of two terms: a linearization of the objective function and a proximity term. 

%multiple gradient updates should be performed 

%In these methods a
%sum of two terms is iteratively being minimized: a linearization of the objective function and a proximity term which
%restricts two consecutive updates to be ‘close’ to each other

%We introduce Mirror Descent Policy Optimization (MDPO), a new Reinforcement Learning (RL) algorithm based on Mirror Descent optimization on the original RL objective. 

%We develop two versions of MDPO, resulting in On-policy and Off-policy variants. We establish connections between On-policy MDPO and Trust Region Policy Optimization methods (i.e. TRPO and PPO), which is followed by an empirical comparison. We then extend Off Policy MDPO to incorporate entropy regularization and show similarities to Soft Actor Critic (SAC). A similar empirical comparison follows and finally, we show that MDPO outperforms or is on-par with the mentioned RL methods when evaluated on the Mujoco domain. In addition, MDPO remains closely attached to the supporting theory and efficient in ease of implementation.  
\end{abstract}



% We develop two versions of MDPO, namely an On-Policy and an Off-Policy variant. We show how popular policy gradient algorithms are related to, and in certain cases, are specific instances of MDPO. Furthermore, to enhance reproducibility, we dissect MDPO's implementation based on the code level optimizations possible, comparing it with its counterparts in various baseline methods. Lastly, we show how entropy regularization can be easily incorporated into MDPO, serving as a bridge to understanding a vast majority of literature on entropy regularized MDPs. MDPO outperforms or is on-par with state-of-the-art RL methods when evaluated on the Mujoco domain, while remaining closely attached to the supporting theory and efficient in ease of implementation.  



==> Sections/Background.tex <==
\vspace{-0.1in}
\section{Preliminaries}
\label{sec:prelim}
\vspace{-0.05in}

In this paper, we assume that the agent's interaction with the environment is modeled as a $\gamma$-discounted Markov decision process (MDP), denoted by $\mathcal{M}=(\mathcal{S}, \mathcal{A},P,R,\gamma,\mu)$, where $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces; $P \equiv P(s'|s,a)$ is the transition kernel; $R \equiv r(s,a)$ is the reward function; %with the maximum value of $R_{\text{max}}$; 
$\gamma\in(0,1)$ is the discount factor; and $\mu$ is the initial state distribution. Let $\pi: \mathcal{S}\rightarrow \Delta_{\mathcal{A}}$ be a stationary Markovian policy, where $\Delta_{\mathcal{A}}$ is the set of probability distributions on $\mathcal{A}$. The discounted frequency of visiting a state $s$ by following a policy $\pi$ is defined as $\rho_\pi(s)\equiv (1-\gamma) \mathbb{E}[\sum_{t\geq 0}\gamma^t \mathbb I \{s_t=s\}| \mu, \pi]$. The value function of a policy $\pi$ at a state $s\in\mathcal{S}$ is defined as $V^\pi(s) \equiv \mathbb{E}[\sum_{t\geq 0}\gamma^tr(s_t,a_t)|s_0=s, \pi]$. Similarly, the action-value function of $\pi$ is defined as $Q^{\pi}(s,a) = \mathbb{E}[\sum_{t\geq 0}\gamma^tr(s_t,a_t)|s_0=s,a_0=a,\pi]$. The difference between the action-value $Q$ and value $V$ functions is referred to as the advantage function $A^{\pi}(s, a) = Q^{\pi}(s, a) - V^{\pi}(s)$. %In all the above definitions, the expectation is over all the randomness in the policy, dynamics, and rewards. %The objective is to find an optimal policy $\pi^*$, i.e.,~a policy with the maximum value at every state.

Since finding an optimal policy for an MDP involves solving a non-linear system of equations and the optimal policy may be deterministic (less explorative), many researchers have proposed to add a regularizer in the form of an entropy term to the reward function, and then solve the entropy-regularized (or {\em soft}) MDP (e.g.,~\cite{Kappen05PI,Todorov06LS,neu2017unified}). In this formulation, the reward function is modified as $r_{\lambda}(s,a) = r(s,a) + \lambda H(\pi(\cdot|s))$, where $\lambda$ is the regularization parameter and $H$ is an entropy-related term, such as Shannon entropy~\cite{fox2015taming,pcl}, Tsallis entropy~\cite{Lee18SM,Nachum18PC}, or relative entropy~\cite{Azar12DP,nachum2017trust}. Setting $\lambda=0$, we return to the original formulation, also referred to as the {\em hard} MDP. In what follows, we use the terms `regularized' and `soft' interchangeably. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.05in}
\subsection{Mirror Descent in Convex Optimization}
\label{subsec:MD}
\vspace{-0.025in}

Mirror Descent (MD)~\cite{beck2003mirror} is a first-order trust-region optimization method for solving constrained convex problems, i.e.,~$x^* \in \argmin_{x\in C} \; f(x)$, 
%
% \vspace{-0.15in}
% \begin{small}
% \begin{equation}
% \label{eq:MD-Opt}
% x^* \in \argmin_{x\in C} \; f(x),    
% \end{equation}
% \end{small}
% \vspace{-0.225in}
%
where $f$ is a convex function and the constraint set $C$ is convex compact. In each iteration, MD minimizes a sum of two terms: {\bf 1)} a linear approximation of the objective function $f$ at the previous estimate $x_k$, and {\bf 2)} a proximity term that measures the distance between the updated $x_{k+1}$ and current $x_k$ estimates. MD is considered a trust-region method, since the proximity term keeps the updates $x_k$ and $x_{k+1}$ close to each other. We may write the MD update as
%
%\vspace{-0.3in}
%\begin{small}
\begin{equation}
\label{eq: md general update}
x_{k+1} \in \argmin_{x \in C} \; \langle \nabla f(x_{k}), x - x_{k} \rangle + \frac{1}{t_k} B_{\psi}(x, x_k), 
\end{equation}
%\end{small}
%\vspace{-0.15in}
%
where \begin{small}$B_{\psi}(x,x_k):= \psi(x) - \psi(x_k) - \langle\nabla\psi(x_k),x-x_k\rangle$\end{small} is the Bregman divergence associated with a strongly convex {\em potential} function $\psi$, and $t_k$ is a step-size determined by the MD analysis. When $\psi = \frac{1}{2} \lVert \cdot \rVert_{2}^{2}$, the Bergman divergence is the Euclidean distance $B_{\psi}(x,x_k)=\frac{1}{2}\lVert x-x_k\rVert_2^2$, and~\eqref{eq: md general update} becomes the {\em projected gradient descent} algorithm~\cite{beck17FO}. When $\psi$ is the negative Shannon entropy, the Bregman divergence term takes the form of the KL divergence, i.e.,~$B_{\psi}(x,x_k)=\text{KL}(x,x_k)$. In this case, when the constraint set $C$ is the unit simplex, $C=\Delta_{\mathcal X}$, MD becomes the {\em exponentiated gradient descent} algorithm and~\eqref{eq: md general update} has the following closed form~\cite{beck2003mirror}:
%
%\vspace{-0.125in}
%\begin{small}
\begin{equation}
x^{i}_{k+1} = \frac{x^{i}_{k}\exp\big(-t_k\nabla_i f(x_k)\big)}{\sum_{j=1}^n x^{j}_{k}\exp\big(-t_k\nabla_j f(x_k)\big)},
\label{closed form}
\end{equation}
%\end{small}
%\vspace{-0.125in}
%
where $x^i_{k}$ and $\nabla_i f$ are the $i^{\text{th}}$ coordinates of $x_k$ and $\nabla f$.

% \manan{\textbf{Insert:} Intro to MD formulation}


==> Sections/Conclusion.tex <==
\vspace{-0.1in}
\section{Conclusions}
\vspace{-0.05in}

We derived on-policy and off-policy algorithms from the theory of MD in RL. Each policy update in our MDPO algorithms is formulated as a trust-region optimization problem. However, our algorithms do not update their policies by solving these problems, instead, update them by taking {\em multiple} gradient steps on the objective function of these problems. We described in detail the relationship between on-policy MDPO and TRPO and PPO. We also discussed how SAC can be derived by slight modifications of off-policy MDPO. Finally, using a comprehensive set of experiments, we showed that on-policy and off-policy MDPO can achieve performance better than or equal to these three popular RL algorithms, and thus can be considered as excellent alternatives to them. %We described the relationship between on-policy MDPO and two popular trust-region RL algorithms: TRPO and PPO, and showed that it performs better than or on par with TRPO and significantly better than PPO across a number of continuous control tasks. We then discussed how the popular SAC algorithm can be derived by slight modifications of off-policy MDPO, and showed that off-policy MDPO performs better than or on par with SAC in these tasks. To summarize, our MDPO algorithms derived from the MD principles, offer a unifying view for a number of popular RL algorithms, and can achieve performance better than or equal to state-of-the-art RL algorithms. 

We can think of several future directions. In addition to evaluating MDPO algorithms in more complex and realistic problems, we would like to see their performance in discrete action problems in comparison with algorithms like DQN and PPO. Investigating the use of Bregman divergences other than KL seems to be promising. Our work with Tsallis entropy is in this direction but more algorithmic and empirical work needs to be done. Finally, there are recent theoretical results on incorporating exploration into the MD-based updates. Applying exploration to MDPO could prove most beneficial, especially in complex environments.

%To conclude, there are several empirical interesting future directions, arising from the theoretical background of MDPO. A possible extension of this work would be testing MDPO in online (adversarial) MDPs, following the roots of MD as an online optimization algorithm. Moreover, using different Bregman divergence than KL and Tsallis can possibly lead to further improvements. Finally, recent theory suggests to incorporate exploration into the MD based updates. Applying exploration to MDPO could prove most beneficial, especially in complex environments.

%In this work, we proposed policy optimization algorithms derived from the theoretical framework of MD applied to the RL objective. We developed two particular variants, on-policy and off-policy {\small MDPO} and showed that they perform better than or on par with popular baseline approaches such as {\small TRPO}, {\small PPO}, and {\small SAC}. Our results reveal the importance of the number of gradient steps used to solve the trust-region problem. Indeed, the theoretical framework of MDPO suggests that ignoring this hyper-parameter results in solving a naive vanilla policy gradient algorithm, instead of the required trust region problem. Moreover, contrary to popular belief, we showed that a hard constraint on the policy update is not a necessity for high performance gains and that an unconstrained method works just as well or better. Overall, we propose a theoretically well motivated algorithm that achieves strong performance, while providing a unified approach to viewing multiple popular RL methods.

% \begin{itemize}
%     \item We achieve better or on par empirical performance when compared to both TRPO and PPO.
%     \item The above is a simpler objective when compared to its TRPO and PPO counter-parts. Precisely, we do not require a natural gradient based update as in TRPO or a clipping based objective as in PPO. 
%     \item The schedule used for adjusting $\eta$ is simple and theoretically grounded. Additionally, we do not pose any specific schedule for the outer learning rate $\eta$. TRPO on the other hand uses a more heuristic approach where the outer learning rate is updated based on the KL term, inducing further complexity in terms of deciding the KL threshold $\delta$. In other words, we do not require a hard constrained update based on a target KL divergence. 
% \end{itemize}

% Alternative conclusions:

% In this work, we proposed the MDPO algorithm, a policy optimization algorithm based on the mirror descent framework. We
% Our empirical study suggests,  

==> Sections/Experiments.tex <==
\vspace{-0.1in}
\section{Experimental Results}
\label{sec:experiments}
\vspace{-0.05in}

%\setlength{\belowcaptionskip}{-20pt}

In this section, we empirically evaluate our on-policy and off-policy MDPO algorithms on a number of continuous control tasks from OpenAI Gym~\cite{brockman2016openai}, and compare them with state-of-the-art baselines: TRPO, PPO, and SAC. We report all experimental details, including the hyper-parameter values used by the algorithms, in Appendix~\ref{app-sec:experiment-detail}. In the tabular results, both in the main paper and in Appendices~\ref{app-sec:on-policy-results} and~\ref{app-sec:off-policy-results}, we report the final training scores averaged over $5$ runs and their $95\%$ confidence intervals (CI). We bold-face the values with the best mean scores.

For off-policy MDPO, we experiment with two potential functions $\psi$ to define the Bregman divergence $B_\psi$: \textbf{1)} Shannon entropy, which results in the KL version (described in Section~\ref{sec:Off-Policy MDPO}), and \textbf{2)} Tsallis entropy, which results in the Tsallis version of off-policy MDPO. We refer the reader to Appendix~\ref{app-sec:Tsallis} for the complete description and detailed derivation of the Tsallis version. Note that we did not pursue a similar bifurcation between Tsallis and KL induced Bregman divergences for the on-policy case since the exact derivations are more tedious there. Another important point to note is that the Tsallis entropy gives us a range of entropies, controlled by the parameter $q \in (0, 2]$ (see Appendix~\ref{app-sec:Tsallis}). Two special cases are {\bf 1)} Shannon entropy for $q=1.0$, and {\bf 2)} sparse Tsallis for $q=2.0$~\cite{Lee18SM,Lee19TR,Nachum18PC}.

%- why not on-policy tsallis
%- tsallis q and its range

%\vspace{-0.175in}

%\setlength{\belowcaptionskip}{10pt}

\begin{comment}
\begin{figure*}[ht]
    \centering
    \tiny
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/Hopper_noent.jpg}
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/Walker_noent.jpg}
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/HalfCheetah_noent.jpg}
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/Ant_noent.jpg}
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/HumanoidStandup_noent.jpg}
    \includegraphics[scale=0.20]{Plots/OnPolicy-Unregularized/Humanoid_noent.jpg} \\
    \includegraphics[scale=0.3]{Plots/OnPolicy-Unregularized/legend-M.jpg}
    \caption{Performance of the multi-step SGD version (MDPO-M), compared against vanilla PPO, TRPO on Hopper-v2, Walker2d-v2, HalfCheetah-v2, Ant-v2, HumanoidStandup-v2 and Humanoid-v2.}
    \label{fig:OnPolicy}
\end{figure*}

%\begin{figure}
%    \centering
    
%    \caption{Performance of off-policy MDPO for different values of $m$ for HalfCheetah-v2.}
%    \label{fig:SGDstep}
%\end{figure}

%\begin{figure*}[ht]
%    \centering
%    \includegraphics[scale=0.20]{Plots/On-vs-Off/HalfCheetah.jpg}
%    \includegraphics[scale=0.20]{Plots/On-vs-Off/Ant.jpg}
%    \includegraphics[scale=0.20]{Plots/On-vs-Off/Humanoid.jpg}
%    \includegraphics[scale=0.3]{Plots/On-vs-Off/legend.jpg} \\
%    \includegraphics[scale=0.20]{Plots/OffPolicy-Regularized-New/HalfCheetah.jpg}
%    \includegraphics[scale=0.20]{Plots/OffPolicy-Regularized-New/Ant.jpg}
%    \includegraphics[scale=0.20]{Plots/OffPolicy-Regularized-New/Humanoid.jpg}
%   \includegraphics[scale=0.3]{Plots/OffPolicy-Regularized-New/legend.jpg}
%    \caption{Performance of off-policy MDPO compared with on-policy MDPO (Top) and soft off-policy MDPO compared with SAC (Bottom) on HalfCheetah-v2, Ant-v2, and Humanoid-v2.}
%    \label{fig:OffPolicy}
%\end{figure*}
\end{comment}

\begin{comment}
\begin{table*}
\centering
\footnotesize
\begin{tabular}{c | c | c | c}\hline
  & MDPO-LOADED & TRPO-LOADED & PPO-LOADED \\ \hline %\hline
 %\rowcolor{Grey}
 Hopper-v2 & \textbf{2318 \tiny(\boldmath$\pm$75)}  & 1941 \tiny($\pm$335)  & 1568 \tiny($\pm$291)  \\
 %\hline
 Walker2d-v2 & \textbf{2967 \tiny(\boldmath$\pm$298)}  & 2882 \tiny($\pm$191)  & 610 \tiny($\pm$115) \\
 %\hline
 %\rowcolor{Grey}
 HalfCheetah-v2 & \textbf{2385 \tiny(\boldmath$\pm$655)}  & 1942 \tiny($\pm$575)  & 659\tiny($\pm$316) \\
 %\hline
 Ant-v2 & \textbf{1845 \tiny(\boldmath$\pm$219)} & 1519 \tiny($\pm$267)  & -164 \tiny($\pm$37) \\
 %\hline
 %\rowcolor{Grey}
 Humanoid-v2 & \textbf{976 \tiny(\boldmath$\pm$143)} & 865 \tiny($\pm$102)  & 468 \tiny($\pm$10) \\
 %\hline
 HumanoidStandup-v2 & \textbf{128221 \tiny(\boldmath$\pm$4532)}  & 116711 \tiny($\pm$1876)  & 70166 \tiny($\pm$2643) \\
 \hline
\end{tabular}
\caption{Averaged cumulative returns for loaded versions of MDPO, TRPO and PPO.}
\label{tab:Exps-Loaded}
\end{table*}
\end{comment}


\begin{comment}
In previous sections, we have established similarities to these methods and therefore, they form a natural baseline for our work. We evaluate all algorithms OpenAI Gym \cite{brockman2016openai} based continuous control tasks, including Hopper-v2, Walker2d-v2, HalfCheetah-v2, Ant-v2, Humanoid-v2 and HumanoidStandup-v2. All experiments are run for 10 million environment time steps, across 5 random seeds. Each plot shows the empirical mean of the random runs while the shaded region represents a 95$\%$ confidence interval. We report results in both figure and tabular forms. The tabular results denote the average performance across the whole training period, i.e. 10M time steps. This allows a comparison between any two methods both in terms final performance and the sample complexity. 

The widely available OpenAI Baselines \cite{dhariwal2017openai} based PPO implementation uses the following five major modifications to the original algorithm presented in \cite{schulman2017proximal} -- value function clipping, reward normalization, observation normalization, orthogonal weight initialization and the Adam optimizer. These are referred to as code level optimization techniques (as mentioned in above sections) and are originally noted in \cite{engstrom2019implementation}. Following the original notation, we refer to the vanilla or minimal version of PPO, i.e. without these modifications as PPO-M. On the other hand, the PPO version including all such code level optimizations, with the hyperparameters given in \cite{schulman2017proximal} is referred to as PPO-LOADED. This version, although being far from the theory, has been shown to be the best performing one, and so forms as a good baseline. We do a similar bifurcation for TRPO and on-policy MDPO. We report all details of our on-policy experiments including hyperparameter values in Table~\ref{tab:Hyperparams-TRPO} of the Appendix.

Similarly, for the off-policy and soft off-policy MDPO versions, we again restrain from using the optimization tricks mentioned above. However we do employ three techniques that are common in actor-critic based algorithms, namely: using separate $Q$ and $V$ functions as in \cite{haarnoja2018soft}, using two $Q$ functions to reduce overestimation bias and using soft target updates for the value function. Prior work \cite{fujimoto2018addressing, lillicrap2015continuous} has shown these techniques help improve stability. Finally, for the soft off-policy MDPO case, we performed a scan over the entropy coefficient and fix $\lambda = 0.1$ across all tasks. For SAC, we use $\lambda = 0.2$ across all tasks, which is the recommended value for most tasks in \cite{haarnoja2018soft}. We report all details of our off-policy experiments including hyperparameter values in Table~\ref{tab:Hyperparams-SAC} of the Appendix. Finally, for all experiments, we use a theoretically motivated schedule for the KL coefficient (see line-\ref{point:tk} in section~\ref{sec : On-Policy MDPO} for details).
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.05in}
\subsection{On Multiple SGD Steps}
\label{subsec:multiple-step-SGD}
\vspace{-0.025in}

In on-policy MDPO, we implement the multi-step update at each MD iteration of the algorithm, by sampling $M$ trajectories from the current policy, generating estimates of the advantage function, and performing $m$ gradient steps using the same set of trajectories. We evaluated on-policy MDPO for different values of $m$ in all tasks. We show the results for Walker2d in Figure~\ref{fig:SGDstep} (top). The results for all tasks show a clear trade-off between $m$ and the performance. Moreover, $m=10$ seems to be the best value across the tasks. This is why we use $m=10$ in all our on-policy MDPO experiments. Our results clearly indicate that using $m=1$ leads to inferior performance as compared to $m=10$, reaffirming the theory that suggests solving the trust-region problem in RL requires taking several gradient steps at each MD iteration. 
\begin{wrapfigure}{r}{0.375\linewidth}
    \centering
    %\begin{subfigure}[t]{0.45\textwidth}
    %    \centering
    \vspace{-0.1in}
    \includegraphics[scale=0.22]{Plots/SGDstep_tradeoff.png} \\
    \includegraphics[scale=0.225]{Plots/SGDstep_tradeoff_legend.png} \\
    \includegraphics[scale=0.22]{Plots/Walker2d_sgd.png} \\ 
    %    \vspace{-3cm}
   
    %\vspace{-0.075in}
    %\end{subfigure}
    %\begin{subfigure}[t]{0.45\textwidth}
    %    \centering
    
    %    \vspace{-2.3cm}
    \includegraphics[scale=0.225]{Plots/offpolicy_sgd_legend.png} 
    %\end{subfigure}
    \vspace{-0.075in}
    \caption{Performance of on-policy (top) and off-policy (bottom) MDPO (code level optimizations included) for different values of $m$ on the Walker2d task.}% X-axis represents time steps in millions.}
    \vspace{-0.2in}
    \label{fig:SGDstep}
    %\vspace{-0.45in}
\end{wrapfigure}
%\vspace{-0.01in}
Finally, we ran a similar experiment for TRPO which shows that performing multiple gradient steps at each iteration of TRPO does not lead to any improvement. In fact our results showed that in some cases, it even leads to worse performance than when performing a single-step update.

%We evaluate on-policy and off-policy MDPO for several values of the number of gradient steps used at each MD iterate, $m$, in Figure~\ref{fig:SGDstep}. The results show a clear trade-off between $m$ and performance. Since $m=10$ seems to be the best value for most environments, we use that to report all our on-policy results. Moreover, we clearly see that using $m=1$ leads to inferior performance as compared to when $m$ is set to 10, reaffirming the theory which suggests that solving the trust-region problem in RL requires taking several gradient steps. Finally, we checked and noticed that just performing multiple gradient steps at each iteration of TRPO does not lead to any improvement. In fact our initial experiments showed that in some cases, it even leads to worse performance than when performing a single-step update.

For off-policy MDPO, performing multiple SGD steps at each MD iteration (Lines~6 to~10 in Algorithm~\ref{alg:MDPO-OffPolicy}) becomes increasingly time-consuming as the value of $m$ grows. This is because off-policy algorithms perform substantially more gradient updates than their on-policy counterparts (a gradient step per environment step vs.~a gradient step per almost $1,000$ environment steps). To address this issue, we resort to staying close to an $m$-step old copy of the current policy, while performing a single gradient update at each iteration of the algorithm. This copy is updated every $m$ iterations with the parameters of the current policy. Our results for the Hopper domain in Appendix~\ref{app-subsec:multistep-update} show that the performance of MDPO can be improved by performing $m$ gradient updates at each iteration, but we omit from performing these experiments at scale because of their unreasonably high wall-clock time. %\mgh{How much the performance of SAC degrades by doing this? How do we still obtain state-of-the-art performance for SAC?} %\lior{google guy reply: note here that the results reported by SAC also use multiple SGD step at each iteration, and that's why some code bases give an enhanced performance for SAC} \manan{Added the above line for addressing this.}. 
Finally, we evaluated off-policy MDPO for different values of $m$ in all tasks and show the results for Walker2d in Figure~\ref{fig:SGDstep} (bottom). %\footnote{Just for this plot, we halve the shaded CI regions, for enhanced visualization of the training curves.}. 
We found it hard to identify a single best value of $m$ for all tasks. However, $m=1000$ had the most reasonable performance across the tasks, and thus, we use it in all our off-policy MDPO experiments. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.05in}
\subsection{On Code-level Optimizations}
\label{subsec:code-level-optimization}
\vspace{-0.025in}

There are certain ``code-level optimization techniques" used in code-bases of TRPO, PPO, and SAC that result in enhanced performance. In~\cite{engstrom2019implementation}, the authors provided a case study of these techniques in TRPO and PPO. We provide a detailed description of these techniques in Appendix~\ref{app-sec:experiment-detail}, and report the performance of the algorithms without these techniques (vanilla or minimal version) and with these techniques (loaded and loaded+GAE versions) in Appendices~\ref{app-sec:on-policy-results} and~\ref{app-sec:off-policy-results}. Note that the loaded+GAE version of TRPO and PPO match their state-of-the-art results in the literature. 

%The results in Table~\ref{tab:Exps-M} are for the loaded implementations of these algorithms, i.e.,~when the code-level optimizations are included, and thus, match their state-of-the-art results in the literature. 

Overall, the key takeaway from our results is that MDPO performs significantly better than PPO and on-par or better than TRPO and SAC, while being much simpler to implement, and more general as being derived from the theory of MD in RL. In the next two sections, we report our main observations from our on-policy and off-policy experiments. 

\renewcommand{\arraystretch}{1.1}
\begin{table*}
\hspace{-0.3in}
%\centering
\scriptsize
%\hspace{-1.8cm}
\begin{minipage}[t]{8cm}
\centering
\begin{tabular}{c  c  c  c} \toprule
 & \makecell{MDPO} & \makecell{TRPO} & \makecell{PPO} \\ \hline \vspace{-0.3cm} \\
 %\rowcolor{Grey}
 Hopper-v2 &  {\bf 2361 \tiny($\pm$ 518)}  & 1979 \tiny($\pm$ 672)   & 2051 \tiny($\pm$ 241)  \\
 %\hline
 Walker2d-v2 &  {\bf 4834 \tiny($\pm$ 607)} & 4473 \tiny($\pm$ 558)  & 1490 \tiny($\pm$ 292)  \\
 %\hline
 %\rowcolor{Grey}
 HalfCheetah-v2 & {\bf 4172 \tiny($\pm$ 1156)}  & 3751 \tiny($\pm$ 910)  & 2041 \tiny($\pm$ 1319)  \\
 %\hline
 Ant-v2 &  {\bf 5211 \tiny($\pm$ 43)}  & 4682 \tiny($\pm$ 278)  &  59 \tiny($\pm$ 133) \\
 %\hline
 %\rowcolor{Grey}
 Humanoid-v2 &  3234 \tiny($\pm$ 566)  & {\bf 4414 \tiny($\pm$ 132)}  & 529 \tiny($\pm$ 47) \\
 %\hline
 H. Standup-v2 & {\bf 155261 \tiny($\pm$ 3898)}  &  149847 \tiny($\pm$ 2632)  & 97223 \tiny($\pm$4479) \\
 \bottomrule
\end{tabular}
\caption*{\hspace{0cm}{\it On-Policy $\;$ (performance reported at 10M timesteps)}} %\vspace{-0.2cm}
\end{minipage}
%\hspace{2cm}
\begin{minipage}[t]{6cm}
\centering
%\vspace{0.15cm}
\begin{tabular}{c  c  c} \toprule
 \makecell{MDPO-KL} & \makecell{MDPO-Tsallis, $q_{\text{best}}$} & \makecell{SAC} \\ \hline \vspace{-0.3cm} \\
 %\rowcolor{Grey}
 {\bf 2428 \tiny($\pm$ 395)}  & {\bf 2428 {\tiny($\pm$ 395)}}, $q$ = 1.0  & 1870 \tiny($\pm$ 404)  \\
 %{\bf 2428 \tiny($\pm$395)}  & {\bf 1882 {\tiny($\pm$650)}}, $q$ =   & {\bf 1870 \tiny($\pm$404)}  \\
 %\hline
 3591 \tiny($\pm$ 366) & {\bf 4028 {\tiny($\pm$ 287)}}, $q$ = 2.0  & 3738 \tiny($\pm$ 312)  \\
 %\hline
 %\rowcolor{Grey}
 11823 \tiny($\pm$ 154)  & 11823 {\tiny($\pm$ 154)}, $q$ = 1.0 & {\bf 11928 \tiny($\pm$ 342)}  \\
 %{\bf 11823 \tiny($\pm$154)}  & 10927 {\tiny($\pm$ 463)}, $q$ =  & {\bf 11928 \tiny($\pm$342)}  \\
 %\hline
 4434 \tiny($\pm$ 749)  & {\bf 5486 {\tiny($\pm$ 737)}}, $q$ = 2.0 & 4989 \tiny($\pm$ 579) \\
 %\hline
 %\rowcolor{Grey}
 5323 \tiny($\pm$ 348)  & {\bf 5611 {\tiny($\pm$ 260)}}, $q$ = 1.2 & 5191 \tiny($\pm$ 312) \\
 %\hline
 143955 \tiny($\pm$ 4499)  &  {\bf 165882 {\tiny($\pm$ 16604)}}, $q$ = 1.4 &  154765 \tiny($\pm$ 11721) \\
 \bottomrule
\end{tabular}
\caption*{\hspace{0.8cm}{\it Off-Policy}}
\end{minipage}
\vspace{0.0cm}
\caption{Averaged (over $5$ runs) cumulative returns for loaded+GAE version of MDPO, TRPO, PPO, and SAC algorithms, together with their $95\%$ confidence intervals. The values with the best mean scores are bold-faced.}%Results when the code-level optimization techniques are added are available in Appendices~\ref{app-sec:on-policy-results} and~\ref{app-sec:off-policy-results} (These scores match with the state of the art results provided by the three baseline methods considered). We report the mean final training scores averaged across 5 training runs and the 95\% confidence interval (CI) region in brackets. The best values with overlapping CIs are bolded.}
\label{tab:Exps-M}
\vspace{-0.2in}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.05in}
\subsection{On-policy Results}
\label{subsection:on-policy-results}
\vspace{-0.025in}

We implemented three versions of on-policy MDPO, TRPO, and PPO: {\bf 1)} the vanilla or minimal version, {\bf 2)} the loaded version in which we add the code-level optimization techniques to these algorithms, and {\bf 3)} the loaded version plus GAE, whose results are reported in Table~\ref{tab:Exps-M}. The results for all three versions are reported in Appendix~\ref{app-sec:on-policy-results}. 

We elicit the following observations from our results. {\bf First,} on-policy MDPO performs better than or on par with TRPO and better than PPO across all tasks. This contradicts the common belief that explicitly enforcing the constraint (e.g.,~through line-search) as done in TRPO is necessary for achieving good performance. {\bf Second,} on-policy MDPO can be implemented more efficiently than TRPO, because it does not require the extra line-search step. Notably, TRPO suffers from scaling issues as it requires computing the correct step-size of the gradient update using a line search, which presents as an incompatible part of the computation graph in popular auto-diff packages, such as TensorFlow. Moreover, MDPO performs significantly better than PPO, while remaining equally efficient in terms of implementation. {\bf Third,} TRPO performs better than PPO consistently, both in the vanilla case and when the code-level optimizations (including GAE) are added to both algorithms. This is in contrast to the common belief that PPO is a better performing algorithm than TRPO. Our observation is in line with what noted in the empirical study of these two algorithms in~\cite{engstrom2019implementation}, and we believe it further reinforces it. Adding code-level optimizations and GAE improve the performance of PPO, but not enough to outperform TRPO, when it also benefits from these additions. Lastly, {\bf fourth,} it was shown in~\cite{wang2019truly} that PPO is prone to instability issues. Our experiments show that this is indeed the case as PPO's performance improves until the standard time-step mark of $1$M, and then decreases in some tasks. For example, in the Ant-v2 domain, both PPO and TRPO get to a similar score (~1000) around the 1M mark but then PPO's performance decreases whereas TRPO continues to increase, as can be seen in Table~\ref{tab:Exps-M} and Appendix~\ref{app-sec:on-policy-results}.

%When run for longer than the usual number of time-steps, our experiments show that this is indeed the case as the performance improves until the standard time-step mark of 1M, and then decreases in some of the tasks. 


%Note that our `vanilla' implementations do not incorporate Generalized Advantage Estimation (GAE) \cite{schulman2015high} in them. This is since we aim to test the most native version of all algorithms. In the case when we do add the code level optimizations and GAE, we do see some improvement in {\small PPO} performance but not enough to beat {\small TRPO}. Although the authors of \cite{engstrom2019implementation} use GAE in their minimal algorithmic implementations, they show a similar trend and our experiments reinforce this observation. 


%Lastly, {\bf 3)} {\small PPO} has recently been shown to be prone to instability issues by \cite{wang2019truly}. When run for longer than the usual number of timesteps (10M), our experiments show that this is indeed the case as the performance improves until the standard timestep mark (1M) and then decreases for some of the tasks considered. 

%\setlength{\belowcaptionskip}{-15pt}
%\setlength{\belowcaptionskip}{10pt}


%\lior{You used here $t_k$ and $\eta^{\text{outer}}$, I think you can just use $\eta$ and $t_k$, or $\eta^{\text{SGD}}$ and $\eta^\text{MD}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.05in}
\subsection{Off-policy Results}
\label{subsection:off-policy-results}
\vspace{-0.025in}

Similar to the on-policy case, we implemented both vanilla and loaded versions of off-policy MDPO and SAC. We report the results of the loaded version in this section (Table~\ref{tab:Exps-M}), and the complete results in Appendix~\ref{app-sec:off-policy-results}. We observe the following from these results. {\bf First,} off-policy MDPO-KL performs on par with SAC across all tasks. {\bf Second,} off-policy MDPO-Tsallis that has an extra hyper-parameter $q$ to tune can outperform SAC across all tasks. We observe that the best performing values of $q$ are different for each domain but always lie in the interval $[1.0, 2.0]$. {\bf Third,} off-policy MDPO results in a performance increase in most tasks, both in terms of sample efficiency and final performance, in comparison to on-policy MDPO. This is consistent with the common belief about the superiority of off-policy to on-policy algorithms. 
%Finally, {\bf third,} we observed best results when the Tsallis $q$ values used for the Bregman regularization and for MDP regularization were kept the same. We report detailed results on off-policy MDPO when different $q$ values are used in Appendix~\ref{app-subsec:different-tsallis}.

Similar to off-policy MDPO, we can incorporate the Tsallis entropy in SAC. In~\cite{Lee19TR}, the authors showed performance improvement over SAC by properly tuning the value of $q$ in SAC-Tsallis. However, in domains like Humanoid-v2 and Ant-v2, they only reported results for the 1M time-step mark, instead of the standard 3M. In our preliminary experiments with SAC-Tsallis in Appendix~\ref{app-subsec:tsallis-sac}, we did not see much improvement over SAC by tuning $q$, unlike what we observed in our MDPO-Tsallis results. More experiments and further investigation are hence needed to better understand the effect of Tsallis entropy (and $q$) in these algorithms.

% Similar to off-policy MDPO, we can incorporate the Tsallis entropy in SAC  for the MDP regularization and refer to this version as SAC-Tsallis~\cite{Lee19TR}. We implemented SAC-Tsallis but did not see much improvement over SAC, unlike the performance improvement between MDPO and MDPO-Tsallis. These results are reported in Appendix~\ref{app-subsec:tsallis-sac}. Note that ~\citet{Lee18SM} also implement SAC-Tsallis but report results only for the 1M timestep mark for domains like the Humanoid-v2, Ant-v2, instead of the standard 3M mark. Their results therefore do not offer a fair comparison to all the methods discussed in this paper.

%The use of a replay buffer helps improve sample efficiency while using a separate function approximator for the critic, i.e. Q function improves the stability. Lastly, {\bf 3)} we see that adding entropy regularization does not lead to huge considerable performance gains against the unregularized versions in most tasks. This highlights that perhaps entropy regularization in SAC is not the main cause for its improved performance, as is also observed in the Appendix results of \cite{haarnoja2018soft}.

%We emphasize another important point here-- since we use the same hyperparameters (ex. entropy parameter $\lambda$) for all tasks, it is conceivable that fine-tuning our algorithms with respect to the task in hand will result in better performance. However, since our aim here is to present the most vanilla versions of all algorithms, we do not use non-standard (ex. \cite{haarnoja2018soft} use larger neural network and batch sizes) or task-dependent hyperparamater values (ex. different $\lambda$ value for each task). We believe presenting the results in such a way allows for understanding the algorithms better.
%\footnotetext{This is why a direct comparison to results presented in \cite{haarnoja2018soft} is not completely fair.}
%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.25]{Plots/OffPolicy-Unregularized/HalfCheetah_noent.jpg} \\
%    \includegraphics[scale=0.25]{Plots/OffPolicy-Unregularized/Ant_noent.jpg} \\
%    \includegraphics[scale=0.3]{Plots/OffPolicy-Unregularized/legend.jpg}
%    \caption{Performance of off-policy MDPO compared with on-policy MDPO (Minimal version) for HalfCheetah-v2 and Ant-v2 environments.}
%    \label{fig:OffPolicy Paper}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.25]{Plots/OffPolicy-Regularized/Hopper.jpg} \\
%    \includegraphics[scale=0.25]{Plots/OffPolicy-Regularized/Walker.jpg} \\
%    \includegraphics[scale=0.3]{Plots/OffPolicy-Regularized/legend.jpg}
%    \caption{Performance of the soft off-policy MDPO compared with Soft Actor-Critic SAC for Hopper-v2 and Walker2d-v2 environments.}
%    \label{fig:Soft Paper}
%\end{figure}

%We also take note of the following modifications to the vanilla version; annealing learning rate, reward normalization, observation normalization, orthogonal initialization of network weights, 

%\begin{figure*}[h]
%    \centering
%    \includegraphics[scale=0.25]{Plots/Baselines/Hopper-v2.jpg}
%    \includegraphics[scale=0.25]{Plots/Baselines/Walker2d-v2.jpg}
%    \includegraphics[scale=0.25]{Plots/Baselines/HalfCheetah-v2.jpg}
%    \includegraphics[scale=0.25]{Plots/Baselines/Swimmer-v2.jpg}
%    \caption{Performance of the three baselines (TRPO, PPO-M, PPO-Paper) on Hopper-v2, Walker2d-v2, HalfCheetah-v2, Swimmer-v2}
%    \label{fig:Baselines}
%\end{figure*}

%\begin{figure*}[h]
%    \centering
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Hopper_noent_klcoeffanneal_samesgdsteps.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Walker_noent_klcoeffanneal_samesgdsteps.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/HalfCheetah_noent_klcoeffanneal_samesgdsteps.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Swimmer_noent_klcoeffanneal_samesgdsteps.jpg}
%    \caption{Performance of TRPO-SGD i.e. solving equation 3 using SGD on Hopper-v2, Walker2d-v2, HalfCheetah-v2, Swimmer-v2. The KL coefficient is annealed from 1 to 0 across the training iterations. A single batch of data is used to calculate the gradient for "samesgdsteps" number of steps.}
%    \label{fig:Baselines}
%\end{figure*}

%\begin{figure*}[h]
%    \centering
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Hopper_noent_loaded.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Walker_noent_loaded.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/HalfCheetah_noent_loaded.jpg}
%    \includegraphics[scale=0.25]{Plots/TRPO-SGD/Swimmer_noent_loaded.jpg}
%    \caption{Performance of TRPO-SGD i.e. solving equation 3 using SGD on Hopper-v2, Walker2d-v2, HalfCheetah-v2, Swimmer-v2. The KL coefficient is annealed from 0 to 1 across the training iterations. A single batch of data is used to calculate the gradient for 5 number of steps. This included the loaded version, i.e. including the 4 PPO tricks and GAE.}
%    \label{fig:Baselines}
%\end{figure*}


%\subsection{Experiment Labels}

%exp1 : [64, 64] - policy size, reward scaling, ent coef = 1 \\
%exp1.5 : [256, 256] - policy size, reward scaling, ent coef = 1 \\ 
%exp2 : [64, 64] - policy size, no reward scaling, ent coef annealed from 0 to 1 \\
%exp2.5 : [256, 256] - policy size, no reward scaling, ent coef annealed from 0 to 1 \\


==> Sections/Introduction.tex <==
\vspace{-0.15in}
\section{Introduction}
\label{sec:intro}
\vspace{-0.05in}

An important class of RL algorithms consider an additional objective in their policy optimization that aims at constraining the consecutive policies to remain close to each other. These algorithms are referred to as \emph{trust region} or \emph{proximity-based}, resonating the fact that they make the new policy to lie within a trust-region around the old one. This class includes the theoretically grounded conservative policy iteration (CPI) algorithm~\cite{kakade2002approximately}, as well as the state-of-the-art deep RL algorithms, such as trust-region policy optimization (TRPO)~\cite{schulman2015trust} and proximal policy optimization (PPO)~\cite{schulman2017proximal}. The main difference between these algorithms is in the way that they enforce the trust-region constraint. TRPO enforces it explicitly through a line-search procedure that ensures the new policy is selected such that its KL-divergence with the old policy is below a certain threshold. PPO takes a more relaxed approach and updates its policies by solving an unconstrained optimization problem in which the ratio of the new to old policies is clipped to remain bounded. It has been shown that this procedure does not prevent the policy ratios to go out of bound, and only reduces its probability~\cite{wang2019truly,engstrom2019implementation}. 

%Many Policy Optimization (PO) based works in Reinforcement Learning (RL) consider an additional surrogate objective which aims at constraining consecutive policies to be close to each other. Such approaches are usually referred to as \emph{trust region} or \emph{proximity-based} methods, resonating the fact that they make the updated policy lie within a trust region around the former policy. Trust region methods in RL are usually motivated by allowing policy improvement in the presence of uncertainty and estimation errors, by using conservative updates \cite{kakade2002approximately,schulman2015trust}. 

Mirror descent (MD)~\cite{blair1985problem,beck2003mirror} is a first-order optimization method for solving constrained convex problems. Although MD is theoretically well-understood in optimization~\cite{beck17FO,hazan2019introduction}, only recently, has it been investigated for policy optimization in RL~\cite{neu2017unified,geist2019theory,liu2019neural,shani2019adaptive}. 
%These results showed that despite the fact that the value function is not convex w.r.t.~the policy, it is still possible to solve the trust-region problem in closed-form in RL. 
%%{\em tabular} RL\YE{is it important to emphasize the tabular?}. %They also provided theoretical guarantees, consistent to those obtained in convex optimization, for the resulting tabular RL algorithms.\YE{suggest to delete this sentence}
Despite the progress made by these results in establishing connections between MD and trust-region policy optimization, there are still considerable gaps between the trust-region RL algorithms that have been theoretically analyzed in their {\em tabular} form ~\cite{shani2019adaptive} and those that are used in practice, such as TRPO and PPO.   

% \YE{Despite the close relation between MD and the popular policy optimization methods nowadays used, there are several differences between the theoretically analyzed algorithms and the ones that are used in practice. In this paper we focus on these gaps and ask
% \begin{center}
%     \emph{are the gaps between MD, TRPO and PPO necessary from practical perspective?}
% \end{center}
% We discover that following more closely the guidelines suggested by MD  results in well performing algorithm, that is easier to implement and with smaller computational complexity in terms of clock time (the last paragraph is not very exact, probably should be replaced)}

%trust-region problem for policy update in RL is not often convex \lior{This sentence is true, but the non-convexity is of the value function with respect to the policy, and it is not directly connected to the kind of algorithm used (whether its trust-region or not)}, it is still possible to solve it in closed-form in the {\em tabular} case. They also provided theoretical guarantees, similar to those obtained in convex optimization, for the resulting tabular RL algorithms. 

%Mirror Descent (MD)~\cite{blair1985problem,beck2003mirror} is a general trust region method that attempts to keep consecutive iterates close to each other. Recently, several authors derived policy optimization methods by applying the framework of MD to the RL objective and supplied theoretical guarantees for such algorithms~\cite{neu2017unified,geist2019theory, liu2019neural,shani2019adaptive}. In the tabular RL case, solving the trust region problem has a closed form solution. However, when the policy is parameterized by a function class, a closed form solution does not usually exist. We test a natural solution to this problem: solving the trust region problem with gradient descent. To this end, we develop a method called Mirror Descent Policy Optimization (MDPO), where we propose and empirically evaluate performing multiple gradient updates at each MD step. We derive on-policy and off-policy variants of {\small MDPO} and perform a thorough empirical evaluation against multiple well established algorithms. 

% In this paper, motivated by the theory of MD in {\em tabular} RL, our goal is to {\bf 1)} derive scaleable and practical RL algorithms from the MD principles, and to {\bf 2)} use the MD theory to better understand and explain the popular trust-region policy optimization methods. Going beyond the tabular case, when the policy belongs to a parametric class, the trust-region problems for policy update in RL cannot be solved in closed-form. We propose an algorithm, called {\bf\em mirror descent policy optimization} (MDPO), that addresses this issue by {\em approximately} solving these trust-region problems via taking multiple gradient steps on their objective functions. We derive {\em on-policy} and {\em off-policy} variants of MDPO (Section~\ref{sec:MDPO-II}). We highlight the connection between on-policy MDPO and TRPO and PPO (Section~\ref{sec:On-Policy MDPO}), and empirically compare it against these algorithms (Section~\ref{subsection:on-policy-results}). Our results on several continuous control tasks from OpenAI Gym~\cite{brockman2016openai} show that on-policy MDPO performs better than or on par with TRPO and better than PPO across all these tasks. We then show that if we define the trust-region w.r.t.~the {\em uniform policy}, instead of the old one, our off-policy MDPO coincides with the popular soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft}. We discuss this connection in details (Section~\ref{sec:Off-Policy MDPO}) and empirically compare these algorithms, showing that off-policy MDPO performs better than or on par with SAC in the same continuous control problems (Section~\ref{subsection:off-policy-results}). 

In this paper, motivated by the theory of MD in {\em tabular} RL, our goal is to derive scaleable and practical RL algorithms from the MD principles, and to use the MD theory to better understand and explain the popular trust-region policy optimization methods. Going beyond the tabular case, when the policy belongs to a parametric class, the trust-region problems for policy update in RL cannot be solved in closed-form. We propose an algorithm, called {\bf\em mirror descent policy optimization} (MDPO), that addresses this issue by {\em approximately} solving these trust-region problems via taking multiple gradient steps on their objective functions. We derive {\em on-policy} and {\em off-policy} variants of MDPO (Section~\ref{sec:MDPO-II}). We highlight the connection between on-policy MDPO and TRPO and PPO (Section~\ref{sec:On-Policy MDPO}), and empirically compare it against these algorithms on several continuous control tasks from OpenAI Gym~\cite{brockman2016openai} (Section~\ref{subsection:on-policy-results}). We then show that if we define the trust-region w.r.t.~the {\em uniform policy}, instead of the old one, our off-policy MDPO coincides with the popular soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft}. We discuss this connection in detail (Section~\ref{sec:Off-Policy MDPO}) and empirically compare these algorithms using the same set of continuous control problems (Section~\ref{subsection:off-policy-results}). 

Our observations on the comparison between the MDPO algorithms and TRPO, PPO, and SAC are a result of extensive empirical studies on different versions of these algorithms (Section~\ref{sec:experiments} and Appendices~\ref{app-sec:on-policy-results} and~\ref{app-sec:off-policy-results}). In particular, we first compare the vanilla versions of these algorithms in order to better understand how the core of these methods work relative to each other. We then add a number of code-level optimization techniques derived from the code-bases of TRPO, PPO, and SAC to these algorithms to compare their best form (those that obtain the best results reported in the literature) against each other. Through comprehensive experiments, we show that on-policy and off-policy MDPO achieve state-of-the-art performance across a number of benchmark tasks, and can be excellent alternatives to popular policy optimization algorithms, such as TRPO, PPO, and SAC. We address the common belief within the community that explicitly enforcing the trust-region constraint is a necessity for good performance in TRPO, by showing that MDPO, a trust-region method based on the MD principles, does not require enforcing a hard constraint and achieves strong performance by solely solving an unconstrained problem. We address another common belief that PPO is a better performing algorithm than TRPO. By reporting results of both the vanilla version and the version loaded with code-level optimization techniques for all algorithms, we show that in both cases, TRPO consistently outperforms PPO. This is in line with some of the findings from a recent study on PPO and TRPO~\cite{engstrom2019implementation}. Finally, we provide an optimization perspective for SAC, instead of its initial motivation as an entropy-regularized {\em (soft)} approximate dynamic programming algorithm.

% We conclude the introduction by summarizing our main algorithmic contributions and important observations elicited from our experiments:

% \textbf{1.} We derive on-policy and off-policy MDPO algorithms. Through comprehensive experiments, we show how they manifest as fundamental algorithms that achieve state-of-the-art performance across a number of benchmark tasks, and can be excellent alternatives to popular policy optimization algorithms, such as TRPO, PPO, and SAC. %Moreover, MDPO offers a coherent view of these algorithms, by unifying them under a single theoretical construct (that of MD).

% \textbf{2.} We address the common belief in the community that explicitly enforcing the trust-region constraint is a necessity for good performance in TRPO, by showing that MDPO, a trust-region method based on the MD principles, does not require enforcing a hard constraint and achieves strong performance by solely solving an unconstrained problem.

% \textbf{3.} We show how SAC, a popular off-policy method, can be derived by slight modifications to off-policy MDPO. This provides an optimization perspective for SAC, instead of its initial motivation as an entropy-regularized {\em (soft)} approximate policy iteration algorithm. %This new view automatically allows us to improve our understanding of existing algorithms that are built over the original SAC motivation.
% %Overall, MDPO offers a unified (optimization) view of a number of popular RL algorithms, such as TRPO, PPO, and SAC.

% \textbf{4.} We address another common belief--- that PPO is a better performing algorithm than TRPO. By reporting results of both the vanilla version and the version loaded with code-level optimization techniques for all algorithms, we show that in both cases, TRPO consistently performs better than PPO. This is in line with some of the findings from a recent case study on PPO and TRPO by~\citet{engstrom2019implementation}.  
%We therefore emphasize how empirically testing algorithms on a level playing field is crucial to not making false observations.

% \textbf{4.} Finally, MDPO offers a coherent view of a number of popular policy optimization algorithms in RL, by unifying them under a single theoretical construct (that of MD). Through our on-policy and off-policy experiments, we show how MDPO manifests as a fundamental algorithm with high practical utility which achieves state-of-the-art performance across a number of benchmark tasks.

%PPO, SAC, and TRPO, are three highly popular algorithms. Although they might appear to be different (due to their names), all three can be thought of instances of MD. Since the three were derived based on heuristics, there are several differences w.r.t. a possible implementation of MD (e.g.,  opposite KL term, different update rule -- as in SAC, not taking into account the KL divergence in a proper manner as in PPO).

% \manan{\textbf{Insert}: 1-2 line introduction to Mirror Descent} yon: what you wrote seems good.


% Para-1 introduces prominent works that solve the trust region problem, with a one line description of what they actually do.

% Para-2 starts by stating that all such approaches are differently motivated and add a lot of heuristic techniques to them. We can look at them through a general theory of MD policy optimization. In this work, we study how we can solve the trust region problem with gradient descent. End by saying how this helps understanding the other methods.

% Para-3 talks about contributions in general ... how the paper is structured, etc. Can shift it to just before section 4 as well.



% {\color{red} Old Intro first part:}

% Policy Optimization (PO) is among the most successfully used methods in Reinforcement Learning (RL)~\cite{peters2008reinforcement,deisenroth2011pilco,lillicrap2015continuous,levine2016end,gu2017deep}. Many PO methods propose directly optimizing the policy based on the gradient of the objective, while constraining the policy updates to be close to each other. This class of algorithms includes Trust Region Policy Optimization (TRPO) \cite{schulman2015trust} and  Proximal Policy Optimization (PPO) \cite{schulman2017proximal}. As will be shown in our paper, methods like Soft Actor Critic (SAC)~\cite{haarnoja2018soft} which are based on Boltzmann policies, are also closely related to trust region methods following the NE-TRPO algorithm in \cite{shani2019adaptive}.

% Although all the above algorithms enjoy comparable empirical success, they appear different at first glance due to how they are motivated, and by the fact each includes multiple heuristic schemes when practically applied. Instead of treating these algorithms as distinct alternatives, understanding the connections between these methods can help to gain insights into developing better and more efficient RL algorithms. This can be achieved by reinterpreting these algorithms through an umbrella approach, that of performing Mirror Descent optimization on the RL objective.



% {\color{red} New Intro first part:}

%Policy Optimization (PO) is among the most successfully used methods in Reinforcement Learning (RL)~\cite{peters2008reinforcement,deisenroth2011pilco,lillicrap2015continuous,levine2016end,gu2017deep}. In this class of algorithms, the policy is directly optimized based on the gradient of the objective. Many works consider an additional surrogate objective which aims at constraining consecutive policies to be close to each other. This approach includes the Trust Region Policy Optimization (TRPO) \cite{schulman2015trust} and Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, among other algorithms, which are usually referred to as \emph{trust region} or \emph{proximity-based} methods, resonating the fact that they make the updated policy lie within a trust region around the former policy.

% The latter technique is usually approached by adding an entropy regularization term which favors stochastic policies. In this approach, a `soft' MDP is solved instead of the original MDP, which is intended to allow better exploration \cite{fox2015taming} and make the learning process `smoother' \cite{dai2017sbeed,Nachum18PC}. While some PO algorithms only consider this technique as an implementation detail \cite{mnih2016asynchronous}, algorithms such as Soft Actor-Critic (SAC) \cite{haarnoja2018soft} directly aims at solving this problem.

% Trust region methods in RL are usually motivated in allowing policy improvement in the presence of uncertainty and estimation errors, by using conservative updates \cite{kakade2002approximately,schulman2015trust}. 
% Yet, this comes in stark contrast to the interpretation of trust region methods in convex optimization. There, they are regarded as iterative gradient based algorithms for optimizing a constraint optimization problem \cite{beck17FO}. 
% Furthermore, although the above algorithms enjoy comparable empirical success, they appear different at first glance
% by the fact each relies on multiple heuristic schemes when practically applied. Thus, using convex optimization to understand the connections between these methods can help to gain insights into developing better and more efficient RL algorithms \cite{shani2019adaptive}. This can be achieved by reinterpreting these algorithms through an umbrella approach, that of performing Mirror Descent optimization on the RL objective.

%Relying on this reasoning~\cite{schulman2015trust} suggested to iteratively solve a constraint optimization problem to assure consecutive policies remain `close' to one another. This, however, comes in stark contrast to the interpretation of trust region methods in convex optimization -- there, an \emph{unconstrained} optimization problem is solved iteratively~\cite{beck17FO}. Recently, several authors derived policy optimization methods by applying the framework of Mirror Descent~\cite{blair1985problem,beck2003mirror} to the RL objective and supplied theoretical guarantees for such algorithms~\cite{neu2017unified,geist2019theory, liu2019neural,shani2019adaptive}. Relying on their theory we test an umbrella approach for performing Mirror Descent optimization on the RL objective when using neural networks as the function approximators.

%Moreover, \cite{cai2019provably} and \cite{efroni2020optimistic} showed model-based Mirror Descent Policy Optimization to be provably efficient when exploration bonus is added.
% Following their approach, in this work, we formulate Mirror Descent policy optimization algorithms techniques while investigating the benefits in doing so and emphasizing important implementation details. 

% Although the above algorithms enjoy comparable empirical success, they appear different at first glance
% % due to how they are motivated, and 
% by the fact each includes multiple heuristic schemes when practically applied. Interestingly, both techniques can be regarded as forms of MDP regularization techniques \cite{geist2019theory}. Specifically, entropy regularization can be seen as keeping a fixed trust region from the uniform policy. Thus, instead of treating these algorithms as distinct alternatives, understanding the connections between these methods can help to gain insights into developing better and more efficient RL algorithms. This can be achieved by reinterpreting these algorithms through an umbrella approach, that of performing Mirror Descent optimization on the RL objective.

% The above algorithms are often derived from slightly different backgrounds, while including use of multiple heuristic schemes in their practical versions. Understanding the connections between these methods can help us gain insights into developing better and more efficient RL algorithms. Although they might appear to be different due to how they are motivated, they can be connected through an umbrella approach, that of performing Mirror Descent optimization on the RL objective.

%In addition, we note that most contemporary approaches tend to differ drastically from each other in terms of their implementation and thus add an unwanted extra layer of complexity in understanding the underlying algorithms~\cite{henderson2018deep, engstrom2019implementation}. In our work, we strip down our method and the corresponding baseline approaches from any differences that may arise due to their implementation. We achieve this by reporting results on the most natural version of all algorithms, excluding any code level optimizations and use of non-standard hyperparameter values. In doing so, we are able to provide a much more coherent understanding of both MDPO and related methods. 

% \manan{This paragraph is still missing emphasis on the novelty of MDPO, why it is different and why that difference is important! Not sure if all this should be in the below para}
% \yon{I think the story of this paper is : solve the trust region problem with gradient descent. This is a one line message and is easy to understand and possibly motivate. + Don't think that this approach was tested.}

 
% Finally, we show that our theoretically supported approach works better than or on par with current on-policy trust region algorithms, TRPO and PPO, despite the fact that MDPO is not based on a constraint optimization procedure, but on solving an unconstrained problem. This greatly reduces the computational complexity, by averting the need to invert a matrix of the parameters space size or approximate it using, for instance, the conjugate gradient method as done in TRPO.

%\manan{The above para simply states how the paper is structured. Now in the below para we can write the main observations we had from following it.}
%We compare off-policy MDPO with on-policy MDPO and observe significant performance improvement for most tasks. The use of entropy regularization has been shown to allow more exploratory behavior through the policy actions \cite{fox2015taming,haarnoja2018soft} and make the learning process `smoother' \cite{dai2017sbeed,Nachum18PC,shani2019adaptive} at the expense of biasing the optimal solution~\cite{dai2017sbeed}. Following this reasoning, we compare both the hard and soft versions of off-policy MDPO with SAC. Surprisingly, our results show that the three algorithms perform similarly, suggesting that the `soft' entropy-regularization mechanism of SAC may not be the reason behind its good performance. \manan{We need to put less stress on the soft part here. Also, the final line is probably not a good conclusion given the context provided in all of the intro section}
%While some PO algorithms only consider this technique as an implementation detail~\cite{mnih2016asynchronous}, algorithms such as Soft Actor-Critic (SAC)~\cite{haarnoja2018soft} directly aim at solving this problem. 
% Indeed, it was recently shown in~\citet{shani2019adaptive}, that using entropy regularization allows faster convergence when used in conjunction with MD based PO updates.

\begin{comment}
We start by deriving a simple, unconstrained, on-policy version of {\small MDPO}, based on the theory presented in \cite{shani2019adaptive}. On-Policy {\small MDPO} is a multi-step gradient based algorithm and thus bears resemblance to {\small TRPO}, {\small PPO} and Natural Policy Gradient (NPG) \cite{kakade2002natural} techniques.
Then, we propose an off-policy version of {\small MDPO} based on an actor critic framework. Off-policy methods are known to be more sample efficient, by allowing to reuse data from a replay buffer, as was observed in~\citet{haarnoja2018soft, lillicrap2015continuous}. Finally, we introduce a soft version of {\small MDPO} by incorporating entropy regularization to off-policy {\small MDPO}, which bears a resemblance to the popular Soft Actor Critic (SAC) algorithm~\cite{haarnoja2018soft}. 

In correspondence to theory, we show that approximately solving the MD based updates requires performing several gradient steps and empirically identify this number as an important hyper parameter. We discuss different design choices such as the distance metric used in the MD update, the use of regularization, which result in various versions of MDPO, some of which present close similarities to prior literature. This is presented in Table~\ref{tab:Algs}. We advice the reader to refer to this table after going through sections~\ref{sec: MDPO} and~\ref{sec:MDPO-II}. 

Our experiments elicit some important results-- 
\begin{itemize}
    \item  Firstly, as a side result, we empirically show that TRPO is a better performing algorithm than PPO, when compared with the same set of code level optimization tricks. This is contrary to popular belief that PPO is superior to TRPO. \lior{If this is a side result, why is it highlighted and is the first thing we mention? It is already known from other papers. It makes the reader think we don't have anything new to say} \manan{That is a bit of an issue but we want to first state this in order to make the second claim complete.}
    \item We show that MDPO performs better or on par with TRPO, and significantly better than PPO. Note that PPO has been known to be a much simpler method to implement than TRPO. The MDPO implementation remains as simple as PPO, thus offering the best of both algorithms. This is since there is no need to perform a line search or invert the Fisher matrix at each iteration, as in TRPO. 
    \item In the off-policy case, our results show that MDPO performs on par or better than SAC, while offering a cleaner, more unifying theory motivating it. Thus, we are able to highlight a diverse set of design choices that lead to different off-policy algorithms. \lior{Here, we should say that our derivation also sheds new understanding on SAC, unifying SAC under the umbrella of trust-region/mirror descent/optimization related deep RL algorithms. I think this is a main contribution of this paper. If you think it does not belong here, this should be written in the paragraph on the organization of this paper} 
\end{itemize}

Together with the theoretical guarantees that our work is based on, these results argue against the common belief that the trust region problem should be solved using a constraint optimization formulation, which is believed to enhance robustness, as claimed in \cite{schulman2015trust}. Instead, it is more natural to follow the unconstrained formulation of MDPO --it is not only well motivated from a theoretical point of view, but, as an additional benefit, it greatly reduces the computational complexity. Similarly for the off-policy case, we highlight how SAC can be considered as a special case of the trust region family of algorithms, and in particular MDPO. In doing so, MDPO serves as a bridge between on-policy and off-policy PO techniques. Through the coherent picture that MDPO builds, along with its strong performance in both on and off-policy cases, we believe it presents itself as a fundamental algorithm in RL.

\lior{It end with our benefits vs. TRPO which neglects our off-policy contribution, and creates confusion regarding our contribution.I think the last paragraph should state that overall we used theory to derive a new competitive algorithm, which is easy to implement and can be both on policy or off-policy. This algorithm has close relations to both TRPO and SAC, and serves as a bridge between on-policy and off-policy policy optimization techniques, showing that all these methods are actually closely related. By this understanding, and by the fact our algorithm is performing well on both occasions, we believe this algorithm to be a fundamental deep RL algorithm.}

\manan{Modified the last para now! Also, mentioned about deriving SAC as a trust region method here.}
\end{comment}

%\begin{enumerate}
%    \item In this work, we implement several instances of MD derived by the theoretical foundations of Sample Based TRPO (TRPO alike), and Uniform TRPO (SAC alike).
%    \item Based on the MD framework, we built a \emph{multi-step gradient based algorithm and identify the number of gradient steps as an important hyper parameter} (this is something to be done of course: i.e., show the performance of the algorithms relatively to different ratio between improvement and evaluation gradient number). Furthermore, we show our theoretically supported approach works better (?) then the current TRPO, PPO, SAC, algortihms. 

% \lior{I would stress the last sentence more, something like: Our paper serves the following goal:  Showing that keeping the algorithms close to theory allows them to perform better. In this aspect we try to separate between two kinds of heuristics: 1) Freedom of choice w.r.t. the implementation of the algorithm. 2) Algorithmic approximations. Our results show that while the former is important and can allow for significant improvement to the performance of MD-like algorithms, the latter should be handled with care: straying away from theory can lead to worse performance.}
%    \item Our TRPO alike algorithm is not based on constraint optimization procedure, but on solving an unconstraint problem. This greatly reduced the computational complexity - we don't need the invert a matrix with size of number of parameters. \lior{Are you sure this is the case in the real implementation of TRPO? refer to appendix C in the original TRPO paper. They approximate this computation so they actually don't really need to inverse a matrix.}
%    \yon{right, the approximate it somehow. Probably it will be the best to measure it by clock times. regardless, it is true we bypass this step which introduces more hyper parametres and computational complexity.}
%\end{enumerate}

%\manan{So I think we should slightly rephrase the three points above. The way I understand them is: 1) Essentially says that all three can be looked at as instances of MD (regularized, unregularized, On-policy, Off-policy) (the experiments corresponding to this section include results on Mujoco with different hyper params of MDPO) 2) Talks about the theoretical differences between MDPO and others (experiments include TRPO, PPO and SAC results on Mujoco) and finally 3) Talks about the implementation differences/advantages between MDPO and others (running time, complexity in implementing etc. for which we can have some experiments but this section might be more text heavy). Adding to these 3, we can also mention a 4th point/contribution, which is our dissection of all algos in terms of their vanilla version and full/loaded/with tricks versions}

%How we plan to demonstrate (1),(2),(3) (fill free to suggest ideas)?
%\begin{enumerate}
%    \item \lior{The first is more of a statement, theory and discussion than something experimental. This relates to the fact that we use the MD nature of the algorithm instead of the hard-constraints, and to the fact that our off-policy method is true to the MD optimization problem, instead of the SAC. The experimental claim here would be the main experimental claim - that our versions work better because of theory + if a discussion on the regularization parameter in the on-policy version of MDPO}
%    \item ...
%    \item \lior{Maybe it is worth keeping record of the KL divergence, to see if truly we keep small KL in our algorithms, as claimed in the empirical ICLR paper. If so, it is not that interestin. But if it happens that our KL are larger, it might be interesting to note. However, I wouldn't put too much effort in this experiment.}
%\end{enumerate}

%\lior{To conclude: 3 graphs: 1) On policy methods comparison. 2) Off policy methods comparison. 3) regularization comparison - in both off-policy and on policy}

\begin{comment}
\begin{table}
%\centering
\footnotesize
%\begin{minipage}[t]{6cm}
\centering
\vspace{0.1cm}
\begin{tabular}{ c | c  c  c }%\hline
% \cline{3-
  \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \makecell{MDPO \\ on-policy} & \makecell{MDPO \\ off-policy} \\ \hline
 %\rowcolor{Grey}
 & \emph{KL$^*$} & \makecell{\phantom{\tiny{Eq.~\eqref{eq:grad0}}}\checkmark \tiny{Eq.~\eqref{eq:grad0}} \\ \tiny{(Similar to KL-PPO)}} & \checkmark \\
 %\rowcolor{Grey}
 \multirow{-2.8}{*}{Bregman} & \emph{Tsallis} & - & \phantom{$^1$}\checkmark$^1$ \\
 \hline
 %\rowcolor{Grey}
 & \emph{No$^*$} & \checkmark & \makecell{ \phantom{\tiny{Eq.~\eqref{eq:off-policy-MDPO-update3}}}\checkmark \tiny{Eq.~\eqref{eq:off-policy-MDPO-update3}} \\ }\\
 %\rowcolor{Grey}
 \multirow{-2}{*}{Regularization} & \emph{Yes} & - & \makecell{\checkmark \\ \tiny{(Similar to SAC)}} \\
 \hline
 %\rowcolor{Grey}
 & \emph{Reverse$^*$}  & \checkmark & \makecell{\checkmark \\ } \\ 
 %\rowcolor{Grey}
 \multirow{-2}{*}{KL Order} & \emph{Forward} & - & \makecell{\tiny{\citet{mei2018exploration}} \\ \tiny{(with regularization)}}\\
 %\hline
\end{tabular}
%\end{minipage}
\vspace{0.5cm}
\caption{Design parameters which lead to various versions of MDPO. $^*$ denotes the default value of each parameter. For example, $^1$ uses the Tsallis based Bregman divergence and the default values for the other two parameters, i.e. no regularization and a reverse KL order.} \manan{I am going to update this table entirely, it's not understandable right now.}
\label{tab:Algs}
\end{table}
\end{comment}


==> Sections/MDPO-OffPolicy.tex <==
\vspace{-0.05in}
\subsection{Off-Policy MDPO} 
\label{sec:Off-Policy MDPO}
\vspace{-0.025in}

In this section, we derive an off-policy RL algorithm based on the MD update rule~\eqref{MD Uniform}. We refer to this as {\em off-policy} MDPO and provide the pseudo-code in Algorithm~\ref{alg:MDPO-OffPolicy} in Appendix~\ref{appsec: pseudocodes}. To emulate the uniform sampling over the state space required by~\eqref{MD Uniform}, Algorithm~\ref{alg:MDPO-OffPolicy} samples a batch of states from a replay buffer $\mathcal{D}$ (Line 4). While this sampling scheme is not truly uniform, it makes the update less dependent on the current policy. Similar to the on-policy case, we write the update rule~\eqref{MD Uniform} for the policy class $\Theta$ as 

\vspace{-0.2in}
\begin{small}
\begin{align}
\label{eq: off-policy-MDPO-optimization}        
\theta_{k+1} \leftarrow \argmax_{\theta\in\Theta} \; \Psi(\theta,\theta_k), \quad\;\; \text{\em where} \quad \Psi(\theta,\theta_k) = \mathbb{E}_{s\sim\mathcal{D}}\Big[\mathbb{E}_{a\sim\pi_\theta}\big[A^{\theta_k}(s, a)\big] - \frac{1}{t_{k}}\text{KL}(s;\pi_\theta,\pi_{\theta_k})\Big].
\end{align}
\end{small}
\vspace{-0.1in}

%
The main idea in Algorithm~\ref{alg:MDPO-OffPolicy} is to estimate the advantage or action-value function of the current policy, $A^{\theta_k}$ or $Q^{\theta_k}$, in an off-policy fashion, using a batch of data randomly sampled from the replay buffer $\mathcal{D}$. In a similar manner to the policy update of our on-policy MDPO algorithm (Algorithm~\ref{alg:MDPO-OnPolicy}), described in Section~\ref{sec:On-Policy MDPO}, we then update the policy by taking multiple SGD steps on the objective function $\Psi(\theta,\theta_k)$ of the optimization problem~\eqref{eq: off-policy-MDPO-optimization} (by keeping $\theta_k$ fixed). Algorithm~\ref{alg:MDPO-OffPolicy} uses two neural networks $V_\phi$ and $Q_\psi$ to estimate the value and action-value functions of the current policy. It then uses them to estimate the advantage function, i.e.,~$A^{\theta_k}\approx Q_\psi^{\theta_k}-V_\phi^{\theta_k}$. The $Q_\psi$ update is done in a $\text{TD}(0)$ fashion, while the $V_{\phi}$ update involves fitting the value function to the $Q_{\psi}$ estimate of the current policy. For policy update, Algorithm~\ref{alg:MDPO-OffPolicy} uses the reparameterization trick and replaces the objective function $\Psi$ in~\eqref{eq: off-policy-MDPO-optimization} with the following loss:
%
%\vspace{-0.2in}
%\begin{small}
\begin{align}
L(\theta,\theta_k) = \mathbb{E}_{\tiny \begin{matrix} {s \! \sim \! \mathcal{D}} \\[-1pt] {\epsilon \! \sim\! \mathcal{N}} \end{matrix}}\big[&\log \pi_\theta\big(\widetilde{a}_\theta(\epsilon,s)|s\big) - \log \pi_{\theta_k}\big(\widetilde{a}_\theta(\epsilon,s)|s\big) - t_k Q^{\theta_k}_\psi\big(s,\widetilde{a}_\theta(\epsilon,s)\big)\big],
\label{eq:off-policy-MDPO-update3}
\end{align}
%\end{small}
%\vspace{-0.1in}
%
where $\widetilde{a}_{\theta} (\epsilon, s)$ is the action generated by sampling the $\epsilon$ noise from a zero-mean normal distribution $\mathcal N$. We can easily modify Algorithm~\ref{alg:MDPO-OffPolicy} to optimize {\em soft} (entropy regularized) MDPs. In this case, in the critic update (Line~12 of Algorithm~\ref{alg:MDPO-OffPolicy}), the $Q_\psi$ update remains unchanged, while in the $V_\phi$ update, the target changes from $\mathbb E_{a\sim\pi_{\theta_{k+1}}}[Q_\psi(\cdot,a)]$ to $\mathbb E_{a\sim\pi_{\theta_{k+1}}}[Q_\psi(\cdot,a)-\lambda\log\pi(a|\cdot)]$. 
%update the reward function is replaced by its soft version $r_\lambda(s,a)=r(s, a) -\lambda\log\pi_\theta(a|s)$. 
The loss function~\eqref{eq:off-policy-MDPO-update3} used for the actor (policy) update (Lines~7-9 of Algorithm~\ref{alg:MDPO-OffPolicy}) is also modified, $Q_\psi$ becomes the soft $Q$-function and a term $\lambda t_k\log \pi_{\theta_k}(\widetilde{a}_\theta(\epsilon,s)|s)$ is added inside the expectation. 


Similarly to on-policy MDPO that has close connection to TRPO and PPO, discussed in Section~\ref{sec:On-Policy MDPO}, off-policy MDPO (Algorithm~\ref{alg:MDPO-OffPolicy}) is related to the popular soft actor-critic (SAC) algorithm~\cite{haarnoja2018soft}. We now derive SAC by slight modifications in the derivation of off-policy MDPO. This gives an optimization interpretation to SAC, which we then use to show strong ties between the two algorithms.

%Now, we discuss their similarities and differences. Specifically, we carefully examine the derivation of off-policy MDPO to reinterpret SAC. Then, we use this new interpretation to show strong ties between the two algorithms.

{\bf Comparison with SAC:} Soft actor-critic is an approximate policy iteration algorithm in soft MDPs. At each iteration $k$, it first estimates the (soft) $Q$-function of the current policy, $Q^{\pi_k}$, and then sets the next policy to the (soft) greedy policy w.r.t.~the estimated $Q$-function as
%
%\vspace{-0.15in}
%\begin{small}
\begin{equation}
\label{eq:soft-greedy-SAC}
\pi_{k+1}(a|s) \leftarrow \exp\big(Q^{\pi_k}(s,a)\big) \; / \; Z^{\text{SAC}}(s),
\end{equation}
%\end{small}
%\vspace{-0.1in}
%
where \begin{small}$Z^{\text{SAC}}(s)=\mathbb{E}_{a\sim\pi_k(\cdot|s)}\big[\exp\big(Q^{\pi_k}(s,a)\big)\big]$\end{small} is a normalization term. However, since tractable policies are preferred in practice, SAC suggests to project the improved policy back into the policy space considered by the algorithm, using the following optimization problem: 
% it is hard to compute $Z^{\text{SAC}}(s)$, 
% \lior{Not sure this claim is accurate. Instead I would write - "to project the improved policy back to the set of policies, SAC suggest the following optimization procedure".
% SAC's explanation word by word: "Since in practice we prefer
% policies that are tractable, we will additionally restrict the
% policy to some set of policies $\Pi$, which can correspond, for
% example, to a parameterized family of distributions such as
% Gaussians. To account for the constraint that $\pi \in \Pi$, we
% project the improved policy into the desired set of policies.
% While in principle we could choose any projection, it will
% turn out to be convenient to use the information projection
% defined in terms of the Kullback-Leibler divergence."} 
% SAC approximates the update~\eqref{eq:soft-greedy-SAC} by computing the next policy as the one with the minimum KL-divergence to the term on the RHS of~\eqref{eq:soft-greedy-SAC}, i.e., 
%
%\vspace{-0.125in}
%\begin{small}
\begin{equation}
%\begin{split}
\label{eq:SAC-update0}
\theta_{k+1} \leftarrow \argmin_{\theta\in\Theta} \; {\mathcal L}^{\text{SAC}}(\theta,\theta_k), \qquad {\mathcal L}^{\text{SAC}}(\theta,\theta_k) = \mathbb{E}_{s \sim \mathcal{D}} \Big[\text{KL}\big(s;\pi_{\theta},{\frac{\exp\big(Q^{\theta_k}(s,\cdot)\big)}{Z^{\text{SAC}}(s)}}\big)\Big].
%\end{split}
\end{equation}
%\end{small}
%\vspace{-0.1in}
%
% \vspace{-0.25in}
% \begin{small}
% \begin{align}
% \label{eq:SAC-update0}
% &\theta_{k+1} \leftarrow \argmin_{\theta\in\Theta} \; {\mathcal L}^{\text{SAC}}(\theta,\theta_k), \nonumber \\
% &{\mathcal L}^{\text{SAC}}(\theta,\theta_k) = \mathbb{E}_{s \sim \mathcal{D}} \Big[\text{KL}\big(s;\pi_{\theta},{\frac{\exp\big(Q^{\theta_k}(s,\cdot)\big)}{Z^{\text{SAC}}(s)}}\big)\Big].
% \end{align}
% \end{small}
% \vspace{-0.25in}
%
This update rule computes the next policy as the one with the minimum KL-divergence to the term on the RHS of~\eqref{eq:soft-greedy-SAC}

Since the optimization problem in~\eqref{eq:SAC-update0} is invariant to the normalization term, unlike~\eqref{eq:soft-greedy-SAC}, the policy update~\eqref{eq:SAC-update0} does not need to compute $Z^{\text{SAC}}(s)$. By writing the KL definition and using the reparameterization trick in~\eqref{eq:SAC-update0}, SAC updates its policy by minimizing the following loss function:   
%
%\vspace{-0.1in}
%\begin{small}
\begin{equation}
\label{eq:SAC-update}
L^\text{SAC}(\theta,\theta_k) = \mathbb{E}_{\tiny \begin{matrix} {s \! \sim \! \mathcal{D}} \\[-1pt] {\epsilon \! \sim\! \mathcal{N}} \end{matrix}}\big[\lambda \log \pi_{\theta}\big(\widetilde{a}_\theta (\epsilon, s)|s\big) - Q^{\theta_k}_\psi\big(s,\widetilde{a}_\theta(\epsilon, s)\big)\big].
\end{equation}
%\end{small}
%\vspace{-0.1in}
%
Comparing the loss in~\eqref{eq:SAC-update} with the one used in off-policy MDPO (Eq.~\ref{eq:off-policy-MDPO-update3}), we notice that despite the similarities, the main difference is the absence of the current policy, $\pi_{\theta_k}$, in the SAC loss function. To explain the relationship between off-policy MDPO and SAC, recall from Section~\ref{subsec:MD} that if the constraint set is the unit simplex, i.e.,~$C=\Delta_{\mathcal X}$, the MD update has the closed-form shown in~\eqref{closed form}. Thus, if the policy class (constraint set) $\Pi$ in the update rule~\eqref{MD Uniform} is the entire space of stochastic policies, then we may write~\eqref{MD Uniform} in closed-form as (see e.g.,~\cite{mei2018exploration,shani2019adaptive}) 
%
%\vspace{-0.025in}
%\begin{small}
\begin{equation}
\label{eq:off-policy-MDPO-update1}
\pi_{k+1}(a|s) \leftarrow \pi_k(a|s) \exp\big(t_kQ^{\pi_k}(s,a)\big)\; / \; Z(s),
\end{equation}
%\end{small}
%\vspace{-0.1in}
%
where \begin{small}$Z(s)=\mathbb{E}_{a\sim\pi_k(\cdot|s)}\big[\exp\big(t_kQ^{\pi_k}(s,a)\big)\big]$\end{small} is a normalization term. The closed-form solution~\eqref{eq:off-policy-MDPO-update1} is equivalent to solving the constrained optimization problem~\eqref{MD Uniform} in two phases (see~\cite{hazan2019introduction}): {\bf 1)} solving the {\em unconstrained} version of~\eqref{MD Uniform} that leads to the numerator of~\eqref{eq:off-policy-MDPO-update1}, followed by {\bf 2)} {\em projecting} this (unconstrained) solution back into the constrained set (all stochastic policies) using the same choice of Bregman divergence (KL in our case), which accounts for the normalization term in \eqref{eq:off-policy-MDPO-update1}. Hence, when we optimize over the parameterized policy space $\Theta$ (instead of all stochastic policies), the MD update would be equivalent to finding a policy $\theta\in\Theta$ with minimum KL-divergence to the solution of the {\em unconstrained} optimization problem obtained in the first phase (the numerator of Eq.~\ref{eq:off-policy-MDPO-update1}).
This leads to the following policy update rule:
%
%Importantly, the first phase is independent of the constraints. Hence, to impose the policy space constraint when optimizing on the parameterized policy space $\Theta$, the mirror descent update consists of finding a policy in $\Theta$ with minimum KL-divergence w.r.t. the closed form solution of the \emph{unconstrained} optimization problem of the first phase. This leads to the following optimization problem,
%
%\vspace{-0.15in}
%\begin{small}
\begin{equation}
\begin{split}
\label{eq:off-policy-MDPO-update2}
&\theta_{k+1} \leftarrow \argmin_{\theta\in\Theta} \; \mathcal L(\theta,\theta_k), \qquad \mathcal L(\theta,\theta_k) = \mathbb{E}_{s \sim \mathcal{D}} \Big[\text{KL}\big(s;\pi_{\theta},{\pi_{\theta_k}\exp(t_k Q^{\theta_k})}\big)\Big].
\end{split}
\end{equation}
%\end{small}
%\vspace{-0.15in}
%
% \vspace{-0.25in}
% \begin{small}
% \begin{align}
% \label{eq:off-policy-MDPO-update2}
% &\theta_{k+1} \leftarrow \argmin_{\theta\in\Theta} \; \mathcal L(\theta,\theta_k), \nonumber \\
% &\mathcal L(\theta,\theta_k) = \mathbb{E}_{s \sim \mathcal{D}} \Big[\text{KL}\big(s;\pi_{\theta},{\pi_{\theta_k}\exp(t_k Q^{\theta_k})}\big)\Big].
% \end{align}
% \end{small}
% \vspace{-0.275in}
%
If we write the definition of KL and use the reparameterization trick in~\eqref{eq:off-policy-MDPO-update2}, we will rederive the loss function~\eqref{eq:off-policy-MDPO-update3} used by our off-policy MDPO algorithm.\footnote{In soft MDPs, $Q^{\pi_k}$ is replaced by its soft version and a term $-\lambda t_k \log\pi_{\theta_k}(a|s)$ is added to the exponential in~\eqref{eq:off-policy-MDPO-update1}. This will result in the same changes in~\eqref{eq:off-policy-MDPO-update2}. Similar to the hard case, applying the reparameterization trick to the the soft version of~\eqref{eq:off-policy-MDPO-update2} gives us the soft version of the loss function~\eqref{eq:off-policy-MDPO-update3}.} Note that both SAC \eqref{eq:SAC-update0} and off-policy MDPO \eqref{eq:off-policy-MDPO-update2} use KL projection to project back to the set of policies. For SAC, the authors argue that any projection can be chosen arbitrarily. However, our derivation clearly shows that the selection of KL projection is dictated by the choice of the Bregman divergence.

As mentioned earlier, the main difference between the loss functions used in the policy updates of SAC~\eqref{eq:SAC-update} and off-policy MDPO~\eqref{eq:off-policy-MDPO-update3} is the absence of the current policy, $\pi_{\theta_k}$, in the SAC's loss function.\footnote{The same difference can also be seen in the policy updates~\eqref{eq:soft-greedy-SAC} and~\eqref{eq:off-policy-MDPO-update1} of SAC and off-policy MDPO.} The current policy, $\pi_{\theta_k}$, appears in the policy update of off-policy MDPO, because it is a trust-region algorithm, and thus, tries to keep the new policy close to the old one. On the other hand, following the original interpretation of SAC as an approximate dynamic programming algorithm, its policy update does not contain a term to keep the new and old policies close to each other. It is interesting to note that SAC's loss function can be re-obtained by repeating the derivation which leads to off-policy MDPO, and replacing the current policy, $\pi_{\theta_k}$, with the {\em uniform policy} in the objective \eqref{eq: off-policy-MDPO-optimization} of off-policy MDPO. Therefore, SAC can be considered as a trust-region algorithm w.r.t.~the uniform policy (or an entropy regularized algorithm). This means its update encourages the new policy to remain {\em explorative}, by keeping it close to the uniform policy. 


% As mentioned earlier, the main difference between the loss functions used in the policy updates of SAC~\eqref{eq:SAC-update} and off-policy MDPO~\eqref{eq:off-policy-MDPO-update3} is the absence of the current policy, $\pi_{\theta_k}$, in the SAC's loss function.\footnote{The same difference can also be seen in the policy updates~\eqref{eq:soft-greedy-SAC} and~\eqref{eq:off-policy-MDPO-update1} of SAC and off-policy MDPO, respectively.} The current policy, $\pi_{\theta_k}$, appears in the policy update of off-policy MDPO, because it is a trust-region algorithm, and thus, tries to keep the new policy close to the old one. On the other hand, following the original SAC interpretation as an approximate policy iteration algorithm, its policy update does not contain a term to keep the new and old policies close to each other.
% It is interesting to note that SAC's loss function can be re-obtained by repeating the derivation which leads to off-policy MDPO, yet replacing the current policy, $\pi_{\theta_k}$, with the {\em uniform policy} in the loss function of off-policy MDPO, or in other words, replacing the KL divergence term in \eqref{MD Sample-based Theta} with the Shannon entropy. Therefore, SAC can be considered as a trust-region algorithm w.r.t.~the uniform policy. This means its update encourages the new policy to remain {\em explorative} (close to the uniform policy). 

%\lior{I've slightly changed this paragraph to explain the regularization perspective that completes the analogy between Mirror Descent (KL regularization) and FTRL (Entropy regularization, can be seen as trust region w.r.t. the uniform policy, but that's just an observation). }

{\bf SAC as FTRL:} The above perspective suggests that both off-policy MDPO and SAC use similar regularization techniques to optimize the policy. This view allows us to regard the {\em hard} version of SAC as an RL implementation of the {\em follow-the-regularized-leader} (FTRL) algorithm. Thus, the equivalency between MD and FTRL (see e.g.,~\cite{hazan2019introduction}) suggests that off-policy MDPO and SAC are in fact closely related and somewhat equivalent. This is further confirmed by our experimental results reported in Section~\ref{subsection:off-policy-results}.
%Thus, we conjecture that SAC's good performance is possibly mainly due to this new perspective on SAC. Note that using the soft versions of MDPO or SAC is orthogonal to this interpretation, and using refined entropy regularization only adds a final boost to their performance. This is confirmed by both in our experiments and in \citet[Appendix E]{haarnoja2018soft}. 


% \paragraph{SAC as FTRL:}{
% The above perspective that views both off-policy MDPO and SAC as trust-region algorithms allows us to regard the {\em hard} version of SAC as an RL implementation of the follow-the-regularized-leader (FTRL) algorithm. Thus, the equivalency between MD and FTRL (see e.g.,~\citealp{hazan2019introduction}) suggests that off-policy MDPO and SAC are in fact closely related and somewhat equivalent. This is further confirmed by our experimental results reported in Section~\ref{subsection:off-policy-results}.}

%\lior{When I've rewritten this section, I tried to rederive SAC from optimization perspective, instead of the RL soft policy iteration explanation. I believe that this understanding is very valuable and thus tried to stress it. Everything seems kind of coherent right now, but we need to make sure that the reader gets the message. Anyway, I think this also belongs to the introduction, not only because its important, but also because it would be easier for the reader to understand our point, if we repeat it throughout the paper}

{\bf Reverse vs.~Forward KL Direction:} Similar to the on-policy case, the {\em mode-seeking} or {\em reverse} direction of the KL term in off-policy MDPO (Eq.~\ref{eq:off-policy-MDPO-update2}) is consistent with that in the MD update rule in convex optimization. With this direction of KL, the optimization problems for policy update in both off-policy MDPO and SAC are invariant to the normalization term $Z(s)$. Thus, these algorithms can update their policies without computing $Z(s)$. In~\cite{mei2018exploration}, the authors proposed an algorithm, called {\em exploratory conservative policy optimization} (ECPO), that resembles our {\em soft} off-policy MDPO, except in the direction of KL. Switching the direction of KL to {\em mean-seeking} or {\em forward} has the extra overhead of estimating the normalization term for ECPO. However, in~\cite{mei2018exploration}, they argue that it results in better performance. They empirically show that ECPO performs better than several algorithms, including one that is close to off-policy MDPO, which they refer to as {\em policy mirror descent} (PMD), and report poor performance for it. We did not use their code-base and exact configuration, but we did not observe such poor performance for our off-policy MDPO. In fact, experimental results of Section~\ref{subsection:off-policy-results} show that off-policy MDPO performs better than or on-par with SAC in six commonly used MuJoCo domains. More experiments and further investigation are definitely required to better understand the effect of the KL direction in MDPO algorithms.

% Finally, note that we use the \emph{reverse} order for the KL divergence in~\eqref{eq:off-policy-MDPO-update2}. As described above, this choice is driven from the MD theory, and allows us to re-derive~\eqref{eq:off-policy-MDPO-update3}. Using instead the \emph{forward} choice of KL, we would end up with the objective described by \citet{mei2018exploration}. However, following such choice would lose the benefits of invariance to the normalization factor and lead to further design complications \cite{mei2018exploration}. Nevertheless, the same branching between forward and reverse KL choices could potentially be done for on-policy {\small MDPO} as well, but we leave that investigation for future work. A concise view of all the different algorithms discussed is provided in Table~\ref{tab:Algs}.

% Although the close relation between MD and policy optimization has been studied, to the best of our knowledge, there is only a single work that empirically studied the practical outcomes of this relation~\cite{mei2018exploration}. This work focuses on the off-policy case and proposes an algorithm, called Exploratory Conservative Policy Optimization (ECPO), that resembles our soft off-policy MDPO algorithm, except in the direction of the KL term. Although changing the direction of KL from mode seeking or \emph{reverse} (used by off-policy {\small MDPO}) to mean seeking or \emph{forward} has the extra overhead of estimating the normalization term (see Eqs.~\ref{eq:off-policy-MDPO-update1} and~\ref{eq:off-policy-MDPO-update2}),~\citet{mei2018exploration} argue that it results in better performance. They show this by comparing {\small ECPO} with a number of algorithms, including one that is close to our off-policy {\small MDPO} and they refer to as Policy Mirror Descent (PMD). They specifically report poor performance for {\small PMD} in their experiments. Although we did not use their code-base and their exact configuration, we did not observe such poor performance for our off-policy {\small MDPO} algorithm (that uses the mode seeking KL direction). In fact, our experimental results in Section~\ref{subsection:off-policy-results} show that off-policy {\small MDPO} performs better than or on-par with {\small SAC} in six commonly used MuJoCo domains. More experiments and further investigation are definitely required to explain this discrepancy and identify the settings suitable for each algorithm.


%The critic $Q_{\phi}$ is updated in a TD(0) like fashion, where we use a separate value function $V$ for the target. We present the detailed version of off-policy MDPO in Algorithm \ref{alg:MDPO-OffPolicy}.

% \vspace{-0.2in}
% \begin{small}
% \begin{align}
% L(\theta,\theta_k) = \mathbb{E}_{\stackrel{s\sim \mathcal{D}}{\epsilon \sim\mathcal{N}}}[\log \pi_{\theta}(\tilde{a}_{\theta} (\epsilon, s) \lvert s) - \log \pi_{\theta_{k}}(\tilde{a}_{\theta} (\epsilon, s) \lvert s))\\
%      & \hspace{1cm} + \lambda \log \pi_{\theta_{k}}(\tilde{a}_{\theta} (\epsilon, s) \lvert s)  - Q_{\psi}(s, \tilde{a}_{\theta} (\epsilon, s)) \Bigr]
%      \label{Soft MDPO}
% \end{align}
% \end{small}
% \vspace{-0.2in}

%Note that the original Mirror Descent update in the regularized case, as derived in \cite{shani2019adaptive}, is the following,:

%\vspace{-0.7cm}

%\begin{equation}
%\begin{array}{cc}
%     & \pi_{k+1} \leftarrow \displaystyle\arg\max_{\pi} \mathbb{E}_{s \sim \rho_{\pi_{k}}} \Bigl[\mathbb{E}_{a \sim \pi} A_{\lambda}^{\pi_{k}}(s, a) \\
%     & \hspace{2cm} - (\frac{1}{t_{k}} - \lambda) \mbox{KL} (\pi, \pi_{k})\Bigr]
%    \label{MD-Reg}
%\end{array}
%\end{equation}

%or, using the closed form version as above:

%\begin{equation}
%    \pi_{k+1}(a\mid s) \leftarrow \frac{\pi_{k}(a\mid s) \ \text{exp}({t_{k}( Q_{\phi}^{\pi_{k}}(s, a) - \lambda \log(\pi_{k}(a\mid s))})}{Z(s)},
%\end{equation}
%where $\lambda$ is the regularization parameter and Q denotes the soft state-action value function, parameterized by $\psi$. 

%We follow the procedure from Section \ref{Off-Policy MDPO} to derive a similar Off-Policy MDPO algorithm for the regularized case and refer to it as Soft Off-Policy MDPO. 

%We minimize the KL divergence between a $\theta$ parameterized policy $\pi_{\theta}$ and the above target density. This results in the following loss function:

%\begin{equation}
%    L_{\pi}(\theta) = \mathbb{E}_{s \sim \mathcal{D}} \left[ \mbox{KL} \left( \pi_{\theta}(\cdot\mid s) \Bigm\lvert\Bigm\rvert \frac{\pi_{k} \ e^{t_{k}( Q^{\pi_{k}}(s, \cdot) - \lambda \log(\pi_{k}(\cdot\mid s) )}}{Z(s)} \right) \right].
%\end{equation}

%In order to minimize $L_{\pi}$, we again use the reparamaterization trick similar which results in the following simplified objective:

%where $\tilde{a}_{\theta} (\epsilon_{t}, s_t)$ represents the action sample computed by sampling $\epsilon$ noise from a normal Gaussian. 

% Again, similar to \cite{haarnoja2018soft}, we use separate Q and V value functions. In particular, the update for $Q_{\psi}$ is based on the following loss function:

% \vspace{-0.2in}
% \begin{small}
% \begin{equation}
%     L_{Q}(\psi) = \mathbb{E}_{s \sim \mathcal{D}} \ \Bigl[\frac{1}{2}(r(s, a) + \gamma V_{\phi}(s') - Q_{\psi}(s, a)] )^2 \Bigr]
% \end{equation}
% \end{small}
% \vspace{-0.2in}

% where V is the soft state value function, parameterized by $\phi$. The update for $V_{\phi}$ is based on the following loss function:

% \vspace{-0.2in}
% \begin{small}
% \begin{equation}
%     L_{V}(\phi) = \mathbb{E}_{s \sim \mathcal{D}} \ \Bigl[\frac{1}{2}(V_{\phi}(s) - Q_{\psi}(s, \pi(s)) + \lambda \log \pi_{\theta}(a | s) )^2 \Bigr],
% \end{equation}
% \end{small}
% \vspace{-0.2in}



%\manan{Eq 10 and 13 are essentially the same, so I think we can skip mentioning the closed form and the KL minimization. Maybe just describe it once at the preliminary section?}



==> Sections/MDPO-OffPolicyBackup.tex <==
% \vspace{-0.1in}
\subsection{Off-Policy MDPO} 
\label{sec:Off-Policy MDPO}
% \vspace{-0.1in}

\begin{algorithm}[ht]
\begin{small}
    \caption{Off-Policy MDPO}
    \label{alg:MDPO-OffPolicy}
    \begin{algorithmic}[1]
        \STATE {\bfseries Initialize} Replay buffer $\mathcal{D}=\emptyset$; $\;$ Policy networks $\pi_{\text{new}}$ and $\pi_{\text{old}}$; $\;$ and Value networks $V_\phi$ and $Q_\psi$; \\
        \FOR{$k =1,\ldots,K$}
            \STATE Take $a_k$ sampled from the current policy $\pi_{\theta_k}$, observe $r_k$ and $s_{k+1}$, and add $(s_k,a_k,r_k,s_{k+1})$ to $\mathcal{D}$;
            \STATE Sample a batch $\{(s_j, a_j, r_j, s_{j+1})\}_{j=1}^N$ from $\mathcal{D}$;
            \STATE {\color{gray}\# Policy update}
            \STATE Set the new policy $\theta_{k+1}$ by performing $m$ policy updates w.r.t.~the objective function $L_{\pi}(\theta, \theta_{k})$;
%            \FOR{$i =0,\ldots,m-1$}
%            \STATE Update $\theta$ w.r.t.~the objective $L(\theta, \theta_{k})$;
%            \ENDFOR
%            \STATE Set the new policy $\theta_{k+1}$ from the above loop;
            \STATE {\color{gray}\# Q and V updates}
            \STATE Update $\phi$ and $\psi$ w.r.t.~the following objective functions: \\ $L_{V_\phi} = \frac{1}{N}\sum_{j=1}^N\big(V_\phi(s_j)-Q_\psi(s_j,\pi_{\theta_{k+1}}(s_j))\big)^2$;
            \\ $L_{Q_\psi} \! = \! \frac{1}{N} \! \sum_{j=1}^N \!\! \big(r(s_j,a_j) + \gamma V_\phi(s_{j+1}) -  Q_\psi(s_j,a_j)\big)^2$;
        \ENDFOR
    \end{algorithmic}
\end{small}    
\end{algorithm}



In the previous section, we derived an on-policy algorithm from the principles of MD in RL. In this section, we show an off-policy RL algorithm based on the mirror descent (MD) update rule~\eqref{MD Uniform}, can be derived from a similar approach as well (see Algorithm~\ref{alg:MDPO-OffPolicy}). We first recall from Section~\ref{subsec:MD} that if the constraint set in MD is the unit simplex, i.e.,~$C=\Delta$, the MD update has a closed from as shown in Eq.~\ref{eq: md general update}. Therefore, if the constraint set in the update rule~\eqref{MD Uniform} is the entire simplex, instead of the considered policy space $\Pi$ (or equivalently $\Theta$), then we can write it in closed form as (see e.g.,~\citet{mei2018exploration,shani2019adaptive}) 

\vspace{-0.3cm}
\begin{small}
\begin{equation}
\label{eq:off-policy-MDPO-update1}
    \pi_{k+1}(a|s) \leftarrow \frac{\pi_k(a|s) \exp\big(t_kQ^{\pi_k}(s,a)\big)}{Z(s)},
\end{equation}
\end{small}
\vspace{-0.3cm}

where $Z(s)=\mathbb{E}_{a\sim\pi_k(\cdot|s)}\big[t_kQ^{\pi_k}(s,a)\big]$ is a normalization term. Now, to impose the policy space constraint, we update the policy by solving the following optimization problem. This also allows avoiding computing (estimating) the normalization term that can be costly when the number of actions is large or infinite. 

\vspace{-0.4cm}
\begin{small}
%\begin{align}
\begin{multline}
\theta_{k+1} \leftarrow \argmin_{\theta\in\Theta} \; L_\pi(\theta,\theta_k), \ L_{\pi}(\theta,\theta_k) \\
=\mathbb{E}_{s \sim \mathcal{D}} \Big[\mbox{KL}\big(s; \pi_{\theta}, \frac{\pi_{\theta_k}\exp\big(t_k Q^{\theta_k}(s,\cdot)\big)}{Z(s)}\big)\Big], \label{eq:off-policy-MDPO-update2}
\end{multline}
%\end{align}
\end{small}
\vspace{-0.3cm}

where $\mathcal D$ is a distribution over the states. In our algorithm, this distribution is defined by the content of the replay buffer. This means that instead of updating the policy by applying~\eqref{eq:off-policy-MDPO-update1}, Eq.~\ref{eq:off-policy-MDPO-update2} updates the policy by finding one in the policy space $\Theta$ with minimum KL distance to the RHS of~\eqref{eq:off-policy-MDPO-update1}. Note that this update is quite similar to the one used by the Soft Actor-Critic (SAC) algorithm~\cite{haarnoja2018soft}. We will further highlight this connection later in this section. 

The main idea in Algorithm~\ref{alg:MDPO-OffPolicy} is to estimate the advantage or action-value function of the current policy, $A^{\theta_k}$ or $Q^{\theta_k}$, in an off-policy fashion, using the content of the replay buffer, $\mathcal{D}$, and then update the policy by taking multiple SGD steps on the policy objective function of~\eqref{eq:off-policy-MDPO-update2} by keeping $\pi_{\theta_k}$ fixed (in a similar manner to the policy update of our on-policy MDPO algorithm, described in Section~\ref{sec : On-Policy MDPO}). Algorithm~\ref{alg:MDPO-OffPolicy} uses two neural networks $V_\phi$ and $Q_\psi$ to estimate the value and action-value functions of the current policy. Note that advantage function is just the difference of these two functions. The $Q_\psi$ update is done in a $\text{TD}(0)$ fashion. For policy update, Algorithm~\ref{alg:MDPO-OffPolicy} uses the reparameterization trick and replaces the objective function $L(\theta,\theta_k)$ in~\eqref{eq:off-policy-MDPO-update2} with

\vspace{-0.3cm}
\begin{small}
\begin{multline}
\label{eq:off-policy-MDPO-update3}
L(\theta,\theta_k) = \mathbb{E}_{\stackrel{s\sim \mathcal{D}}{\epsilon \sim\mathcal{N}}}\big[\log \pi_\theta\big(\tilde{a}_\theta(\epsilon,s)|s\big) - \log \pi_{\theta_k}\big(\tilde{a}_\theta(\epsilon,s)|s\big) \\
- t_k Q^{\theta_k}_\psi\big(s,\tilde{a}_\theta(\epsilon,s)\big)\big], %\nonumber
\end{multline}
\end{small}
\vspace{-0.3cm}

where $\tilde{a}_{\theta} (\epsilon, s)$ represents the action generated by $\epsilon$ sampled from the zero-mean normal distribution $\mathcal N$. We can easily modify Algorithm~\ref{alg:MDPO-OffPolicy} to optimize {\em soft} (entropy regularized) MDPs, described in Section~\ref{sec:prelim}. In this case, the $V_\phi$ update (Line~8 of Alg.~\ref{alg:MDPO-OffPolicy}) remains unchanged, while in the $Q_\psi$ update the reward function is replaced by its soft version $r_\lambda(s,a)=r(s, a) -\lambda\log\pi_\theta(a|s)$. The policy update of~\eqref{eq:off-policy-MDPO-update3} is also modified by adding a term $\lambda t_k\log \pi_{\theta_k}(\tilde{a}_\theta(\epsilon,s)|s)$ inside the expectation. 

Also note that the we use the \emph{reverse} order for the KL divergence in ~\eqref{eq:off-policy-MDPO-update1}. It is important to realize that this KL choice is independent of the kinds of Bregman divergences one would want to consider, as mentioned in earlier sections. Moreover, with the \emph{reverse} choice of KL, we can get to ~\eqref{eq:off-policy-MDPO-update2}, which was easily derivable directly from the on-policy update rule in~\eqref{MD Sample-based Theta}, when using a replay buffer to sample states from. If we use the \emph{forward} choice of KL here, we would end up with the objective described by \citet{mei2018exploration}. The same branching between forward and reverse KL choices could potentially be done for on-policy {\small MDPO} as well, but we leave that investigation for future work. A concise view of all the different algorithms discussed is provided in Table~\ref{tab:Algs}.

%The critic $Q_{\phi}$ is updated in a TD(0) like fashion, where we use a separate value function $V$ for the target. We present the detailed version of off-policy MDPO in Algorithm \ref{alg:MDPO-OffPolicy}.

% \vspace{-0.2in}
% \begin{small}
% \begin{align}
% L(\theta,\theta_k) = \mathbb{E}_{\stackrel{s\sim \mathcal{D}}{\epsilon \sim\mathcal{N}}}[\log \pi_{\theta}(\tilde{a}_{\theta} (\epsilon, s) \lvert s) - \log \pi_{\theta_{k}}(\tilde{a}_{\theta} (\epsilon, s) \lvert s))\\
%      & \hspace{1cm} + \lambda \log \pi_{\theta_{k}}(\tilde{a}_{\theta} (\epsilon, s) \lvert s)  - Q_{\psi}(s, \tilde{a}_{\theta} (\epsilon, s)) \Bigr]
%      \label{Soft MDPO}
% \end{align}
% \end{small}
% \vspace{-0.2in}

%Note that the original Mirror Descent update in the regularized case, as derived in \cite{shani2019adaptive}, is the following,:

%\vspace{-0.7cm}

%\begin{equation}
%\begin{array}{cc}
%     & \pi_{k+1} \leftarrow \displaystyle\arg\max_{\pi} \mathbb{E}_{s \sim \rho_{\pi_{k}}} \Bigl[\mathbb{E}_{a \sim \pi} A_{\lambda}^{\pi_{k}}(s, a) \\
%     & \hspace{2cm} - (\frac{1}{t_{k}} - \lambda) \mbox{KL} (\pi, \pi_{k})\Bigr]
%    \label{MD-Reg}
%\end{array}
%\end{equation}

%or, using the closed form version as above:

%\begin{equation}
%    \pi_{k+1}(a\mid s) \leftarrow \frac{\pi_{k}(a\mid s) \ \text{exp}({t_{k}( Q_{\phi}^{\pi_{k}}(s, a) - \lambda \log(\pi_{k}(a\mid s))})}{Z(s)},
%\end{equation}
%where $\lambda$ is the regularization parameter and Q denotes the soft state-action value function, parameterized by $\psi$. 

%We follow the procedure from Section \ref{Off-Policy MDPO} to derive a similar Off-Policy MDPO algorithm for the regularized case and refer to it as Soft Off-Policy MDPO. 

%We minimize the KL divergence between a $\theta$ parameterized policy $\pi_{\theta}$ and the above target density. This results in the following loss function:

%\begin{equation}
%    L_{\pi}(\theta) = \mathbb{E}_{s \sim \mathcal{D}} \left[ \mbox{KL} \left( \pi_{\theta}(\cdot\mid s) \Bigm\lvert\Bigm\rvert \frac{\pi_{k} \ e^{t_{k}( Q^{\pi_{k}}(s, \cdot) - \lambda \log(\pi_{k}(\cdot\mid s) )}}{Z(s)} \right) \right].
%\end{equation}

%In order to minimize $L_{\pi}$, we again use the reparamaterization trick similar which results in the following simplified objective:

%where $\tilde{a}_{\theta} (\epsilon_{t}, s_t)$ represents the action sample computed by sampling $\epsilon$ noise from a normal Gaussian. 

% Again, similar to \cite{haarnoja2018soft}, we use separate Q and V value functions. In particular, the update for $Q_{\psi}$ is based on the following loss function:

% \vspace{-0.2in}
% \begin{small}
% \begin{equation}
%     L_{Q}(\psi) = \mathbb{E}_{s \sim \mathcal{D}} \ \Bigl[\frac{1}{2}(r(s, a) + \gamma V_{\phi}(s') - Q_{\psi}(s, a)] )^2 \Bigr]
% \end{equation}
% \end{small}
% \vspace{-0.2in}

% where V is the soft state value function, parameterized by $\phi$. The update for $V_{\phi}$ is based on the following loss function:

% \vspace{-0.2in}
% \begin{small}
% \begin{equation}
%     L_{V}(\phi) = \mathbb{E}_{s \sim \mathcal{D}} \ \Bigl[\frac{1}{2}(V_{\phi}(s) - Q_{\psi}(s, \pi(s)) + \lambda \log \pi_{\theta}(a | s) )^2 \Bigr],
% \end{equation}
% \end{small}
% \vspace{-0.2in}

{\bf Comparison with SAC:} The update rules of our hard and soft off-policy {\small MDPO} algorithms resemble those used by DDPG~\cite{lillicrap2015continuous} and {\small SAC}~\cite{haarnoja2018soft}, respectively. The main difference with {\small SAC} is the absence of the current policy, $\pi_{\theta_k}$, in its policy update, compared to ours shown by Eqs.~\ref{eq:off-policy-MDPO-update1} and~\ref{eq:off-policy-MDPO-update2}. To be more precise, the policy update in {\small SAC} is of the form 

\vspace{-0.3cm}
\begin{small}
\begin{equation}
    L_{\pi}^\text{SAC}(\theta,\theta_k) = \mathbb{E}_{\stackrel{s\sim \mathcal{D}}{\epsilon \sim\mathcal{N}}}\big[\lambda \log \pi_{\theta}\big(\tilde{a}_\theta (\epsilon, s)|s\big) - Q^{\theta_k}_\psi\big(s,\tilde{a}_\theta(\epsilon, s)\big)\big],
    \label{SAC}
\end{equation}
\end{small}
\vspace{-0.3cm}

which clearly shows the absence of $\log\pi_{\theta_k}$, from the {\small MDPO} update rule~\eqref{eq:off-policy-MDPO-update2}. This absence is mainly due to the fact that the {\small SAC} update does not contain a term that keeps the new policy close to the old one. Instead its update encourages the new policy to stay close to the \emph{uniform policy} (remain explorative), and thus, {\small SAC} can be considered as a trust region algorithm w.r.t.~the uniform policy.

%\manan{Eq 10 and 13 are essentially the same, so I think we can skip mentioning the closed form and the KL minimization. Maybe just describe it once at the preliminary section?}



==> Sections/MDPO-OnPolicy.tex <==
\vspace{-0.1in}
\section{Mirror Descent Policy Optimization}
\label{sec:MDPO-II}
\vspace{-0.05in}

In this section, we derive {\em on-policy} and {\em off-policy} RL algorithms based on the MD-style update rules~\eqref{MD Uniform} and~\eqref{MD Sample-based}. We refer to our algorithms as {\em mirror descent policy optimization} (MDPO). Since the trust-region optimization problems in the update rules~\eqref{MD Uniform} and~\eqref{MD Sample-based} cannot be solved in closed-form, we approximate these updates with multiple steps of stochastic gradient descent (SGD) on the objective functions of these optimization problems. In our {\em on-policy} MDPO algorithm, described in Section~\ref{sec:On-Policy MDPO}, we use the update rule~\eqref{MD Sample-based} and compute the SGD updates using the Monte-Carlo (MC) estimate of the advantage function $A^{\pi_k}$ gathered by following the current policy $\pi_k$. On the other hand, our {\em off-policy} MDPO algorithm, described in Section~\ref{sec:Off-Policy MDPO}, is based on the update rule~\eqref{MD Uniform} and calculates the SGD update by estimating $A^{\pi_k}$ using samples from a replay buffer.

In our MDPO algorithms, we define the policy space, $\Pi$, as a class of smoothly parameterized stochastic polices, i.e.,~$\Pi=\{\pi(\cdot|s;\theta):s\in\mathcal S,\theta\in\Theta\}$. We refer to $\theta$ as the policy parameter. We will use $\pi$ and $\theta$ to represent a policy, and $\Pi$ and $\Theta$ to represent the policy space, interchangeably.

%Considering the above theoretical results on using MD update rule to optimize RL objectives, together with some empirical work in this area (e.g.,~\citet{nachum2017trust,mei2018exploration}), led us to derive RL algorithms based on the MD update rules~\eqref{MD Uniform} and~\eqref{MD Sample-based}. We refer to these algorithms as MD policy optimization (MDPO). Since the trust region problem cannot be solved exactly, we resolve to solving it approximately using SGD. Therefore, at each iteration, we perform multiple steps of stochastic gradient descent. We also segregate MDPO in two methods, based on the above two RL formulations. Specifically, in our {\em on-policy} MDPO algorithm, described in Section~\ref{sec : On-Policy MDPO}, we use the update rule~\eqref{MD Sample-based} and perform the updates using Monte-Carlo estimates of $A^{\pi_k}$ gathered by following the current policy, $\pi_k$. Our {\em off-policy} MDPO algorithm, described in Section~\ref{Off-Policy MDPO}, is based on the update rule~\eqref{MD Uniform}, uses samples from a replay buffer to estimate $A^{\pi_k}$ and then performs the update to optimize the policy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vspace{-0.1in}
%\clearpage
\subsection{On-Policy MDPO}
\label{sec:On-Policy MDPO}
\vspace{-0.05in}

In this section, we derive an on-policy RL algorithm based on the MD-based update rule~\eqref{MD Sample-based}, whose pseudo-code is shown in Algorithm~\ref{alg:MDPO-OnPolicy} in Appendix~\ref{appsec: pseudocodes}. %We define our policy space, $\Pi$, as a class of smoothly parameterized stochastic polices $\Pi=\{\pi(\cdot|s;\theta),s\in\mathcal S,\theta\in\Theta\}$. From now on, we will use $\pi$ and $\theta$ to represent a policy, and $\Pi$ and $\Theta$ to represent the policy class, interchangeably. 
%Therefore, we can write the MD update rule~\eqref{MD Sample-based} as
We refer to this algorithm as {\em on-policy} MDPO. We may write the update rule~\eqref{MD Sample-based} for the policy space $\Theta$ (defined above) as

\vspace{-0.2in}
\begin{small}
\begin{align}
\label{MD Sample-based Theta}        
\theta_{k+1} \leftarrow \argmax_{\theta\in\Theta} \; \Psi(\theta,\theta_k), \quad\; \text{\em where} \quad
\Psi(\theta,\theta_k) =\mathbb{E}_{s\sim\rho_{\theta_k}}\Big[\mathbb{E}_{a\sim\pi_\theta}\big[A^{\theta_k}(s, a)\big] - \frac{1}{t_{k}}\text{KL}(s;\pi_\theta,\pi_{\theta_k})\Big].
\end{align}
\end{small}
\vspace{-0.15in}

Each policy update in~\eqref{MD Sample-based Theta} requires solving a constrained (over $\Theta$) optimization problem. In on-policy MDPO, instead of solving this problem, we update the policy by performing multiple SGD steps on the objective function $\Psi(\theta,\theta_k)$. Interestingly, performing only a single SGD step on $\Psi(\theta,\theta_k)$ is not sufficient as $\nabla_\theta\text{KL}(\cdot;\pi_\theta,\pi_{\theta_k})\vert_{\theta=\theta_k}=0$, and thus, if we perform a single-step SGD, i.e.,
%there is no contribution from the KL-term in a single step of SGD, i.e., 
%
%\vspace{-0.15in}
%\begin{small}
\begin{equation*}
\nabla_\theta \Psi(\theta,\theta_k)\vert_{\theta=\theta_k} = \mathbb{E}_{\stackrel{s \sim \rho_{\theta_{k}}}{a \sim \pi_\theta}}\big[\nabla\log\pi_{\theta_k}(a|s)A^{\theta_{k}}(s, a)\big],
\end{equation*}
%\end{small}
%\vspace{-0.16in}
%
the resulting algorithm would be equivalent to {\em vanilla policy gradient} and misses the entire purpose of enforcing the trust-region constraint. As a result, the policy update at each iteration $k$ of on-policy MDPO involves $m$ SGD steps as
%
%\vspace{-0.22in}
%\begin{small}
\begin{align*}
\theta_k^{(0)}=\theta_k, \quad\;\;\; \text{for } \;\; i=0,\ldots,m-1, 
\quad\;\;\; \theta_k^{(i+1)} \leftarrow \theta_k^{(i)} + \eta \nabla_\theta\Psi(\theta,\theta_k)\lvert_{\theta=\theta_k^{(i)}}, \quad\;\;\; \theta_{k+1}=\theta_k^{(m)}, 
\end{align*}
%\end{small}
%\vspace{-0.22in}
%
where the gradient of the objective function 

\vspace{-0.15in}
\begin{small}
\begin{align}
\hspace{-0.125in}\nabla_\theta\Psi(\theta,\theta_k)&\vert_{\theta=\theta_k^{(i)}} = \mathbb{E}_{\tiny\begin{matrix} {s \! \sim \! \rho_{\theta_k}} \\[-1pt] {a\! \sim \! \pi_{\theta_k}} \end{matrix}}\Big[\frac{\pi_{\theta_k}^{(i)}}{\pi_{\theta_k}}\nabla\log\pi_{\theta_k^{(i)}}(a|s)A^{\theta_k}(s,a)\Big] - \frac{1}{t_k}\mathbb{E}_{s\sim\rho_{\theta_k}}\left[\left.\nabla_\theta\text{KL}(s;\pi_\theta,\pi_{\theta_k})\right\vert_{\theta=\theta_k^{(i)}}\right]
\label{eq:grad0}
\end{align}
\end{small}
\vspace{-0.1in}

%\vspace{-0.3cm}
%
can be estimated in an {\em on-policy} fashion using the data generated by the current policy $\pi_{\theta_k}$. Since in practice, the policy space is often selected as Gaussian, we use the closed-form of $\text{KL}$ in this estimation. Our on-policy MDPO algorithm (Algorithm~\ref{alg:MDPO-OnPolicy}, Appendix~\ref{appsec: pseudocodes}) has close connections to two popular on-policy trust-region RL algorithms: TRPO~\cite{schulman2015trust} and PPO~\cite{schulman2017proximal}. We now discuss the similarities and differences between on-policy MDPO and these algorithms.   

%\vspace{-10pt}

% propose to solve this optimization problem (Eq.~\ref{MD Sample-based Theta})

% a practical on-policy algorithm based on the MD update presented in Section \ref{sec: MDPO}. In particular, we propose to solve \ref{MD Sample-based} in an on-policy fashion using multiple steps of Stochastic Gradient Descent (SGD) over the combined objective, while keeping $\pi_{k}$ fixed. To realize this, we first note that performing a single gradient descent step to the objective in \ref{MD Sample-based} results in the following parameter update, where the policy is parameterized as $\pi_{\theta}$ with parameter $\theta$: \lior{Should we explain here the MD like update of the weights? why do we do that?}
% % \vspace{-0.3cm}
% \begin{equation}
%     \theta_{k+1} \leftarrow \displaystyle\arg\max_{\theta} \langle \nabla\Psi(\theta_{k}), \theta - \theta_{k} \rangle - \frac{1}{\eta} \lVert \theta - \theta_{k} \rVert_{2}^{2},
%     \label{One step SGD}
% \end{equation}
% where $\nabla \Psi(\theta_{k}) = \mathbb{E}_{s \sim \rho_{\pi_{\theta_{k}}}} [\mathbb{E}_{a \sim \pi_{\theta_{k}}} \nabla \log\pi_{\theta_{k}} A^{\pi_{\theta_{k}}}(s, a)]$. Notice that there is no gradient contribution from the KL term. This is since gradient of $\mbox{KL}(\pi_{\theta}, \pi_{\theta_{k}})$ evaluated at $\theta = \theta_k$ is 0. This is exactly the vanilla policy gradient update. Therefore, in order to truly incorporate the gradient contribution due to the KL term, \emph{multiple gradient updates} should be done while keeping $\theta_{k}$ fixed. We therefore propose the following multi-step gradient update:

% \begingroup
% \large
% \begin{equation}
% \begin{array}{cc}
%     & \hspace{-4mm} \theta_{i+1} \leftarrow \theta_{i} + \eta g_{i}, \ \ \tiny{i = 1,\ldots,m} \\ \\
%     & \hspace{-6mm} g_{i} = \mathbb{E}_{s \sim \rho_{\pi_{\theta_{k}}}, a \sim \pi_{\theta_{k}}} \nabla_{\theta} \Bigl[\frac{\pi_{\theta}}{\pi_{\theta_{k}}} A^{\pi_{\theta_{k}}}(s, a) - \frac{1}{t_{k}} \mbox{KL} (\pi_{\theta}, \pi_{\theta_{k}}) \Bigr]  \hspace{-1.5mm} \Bigm\lvert_{\theta = \theta{i}},
%     \label{MD-TRPO}
% \end{array}
% \end{equation}
% \endgroup

% \begin{small}
% \begin{align}
%     &\theta_{i+1} \leftarrow \theta_{i} + \eta g_{i}, \quad i = 1,\ldots,m \\ 
% &g_{i} = \mathbb{E}_{s \sim \rho_{\pi_{\theta_{k}}}, a \sim \pi_{\theta_{k}}} \nabla_{\theta} \Bigl[\frac{\pi_{\theta}}{\pi_{\theta_{k}}} A^{\pi_{\theta_{k}}}(s, a) - \frac{1}{t_{k}} \mbox{KL} (\pi_{\theta}, \pi_{\theta_{k}}) \Bigr]  \hspace{-1.5mm} \Bigm\lvert_{\theta = \theta{i}}, \nonumber \\
%     \label{MD-TRPO}
% \end{align}
% \end{small}

% where $m$ is the number of gradient steps taken for solving the $k^{\text{th}}$ MD iterate and $\theta_1$ is set to the current policy's parameters, i.e. $\theta_k$. The policy parameters obtained after solving one MD iterate approximately correspond to $\theta_{k+1}$. We present the detailed version of on-policy MDPO in Algorithm \ref{alg:MDPO=OnPolicy}. 

{\bf Comparison with TRPO:} At each iteration $k$, TRPO considers the constrained optimization problem
%
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
%
%
\vspace{-0.125in}
%\begin{small}
\begin{equation}
\begin{split}
\label{eq:TRPO-update}
&\max_{\theta\in\Theta} \; \mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\Big[\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)}A^{\theta_k}(s,a)\Big], \quad\text{s.t. } \qquad \mathbb{E}_{s\sim\rho_{\theta_k}}\big[\text{KL}(s;\pi_{\theta_{k}}, \pi_{\theta})\big] \leq \delta, 
\end{split}
\end{equation}
%\end{small}
%\vspace{-0.1in}
%
% \vspace{-0.25in}
% \begin{small}
% \begin{align}
% \label{eq:TRPO-update}
% &\max_{\theta\in\Theta} \; \mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\Big[\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)}A^{\theta_k}(s,a)\Big], \\ 
% &\quad\text{s.t. } \qquad \mathbb{E}_{s\sim\rho_{\theta_k}}\big[\text{KL}(s;\pi_{\theta_{k}}, \pi_{\theta})\big] \leq \delta, \nonumber    
% \end{align}
% \end{small}
% \vspace{-0.275in}
%
and updates its policy parameter by taking a step in the direction of the {\em natural gradient} of the objective function in~\eqref{eq:TRPO-update} as \begin{small}$\theta_{k+1} \!\leftarrow\! \theta_k + \eta F^{-1}\mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\big[\nabla\log\pi_{\theta_k}(a|s)A^{\theta_k}(s,a)\big]$\end{small}, 
% \vspace{-0.25in}
% \begin{small}
% \begin{equation*}
% \theta_{k+1} \leftarrow \theta_k + \eta F^{-1}\mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\big[\nabla\log\pi_{\theta_k}(a|s)A^{\theta_k}(s,a)\big],
% \end{equation*}
% \end{small}
% \vspace{-0.225in}
where \begin{small}$F=\mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\left[\nabla\log\pi_{\theta_k}(a|s)\nabla\log\pi_{\theta_k}(a|s)^\top\right]$\end{small} is the {\em Fisher information matrix} for the current policy $\pi_{\theta_k}$. %\footnote{The natural gradient is the result of adding a KL term to the objective function in~\ref{eq:TRPO-update} and then replacing it with its Taylor series expansion.} 
It then explicitly enforces the trust-region constraint in~\eqref{eq:TRPO-update} by a {\em line-search}: computing the KL-term for $\theta=\theta_{k+1}$ and checking if it is larger than the threshold $\delta$, in which case, the step size is reduced until the constraint is satisfied. 


%This update is followed by strictly enforcing the trust region constraint, which is done by computing the KL-term in~\eqref{eq:TRPO-update}, for $\theta=\theta_{k+1}$, and checking if it is larger than the threshold $\delta$. If this is the case, the step size is reduced until the constraint is satisfied. %Note that since the policies are Gaussian, TRPO computes the KL-term in closed-form.

%\lior{Maybe refer to the connection between the natural gradient and MD: https://arxiv.org/pdf/1310.7780.pdf}
\begin{comment}
\begin{minipage}[t]{6cm}%6cm <========================================== 
\begin{algorithm}[H]
\begin{small}
    \caption{On-Policy MDPO}
    \label{alg:MDPO=OnPolicy}
    \begin{algorithmic}[1]
        \STATE {\bfseries Initialize} $V$-network $V_{\phi}$, Policy networks $\pi_{\text{new}}$ and $\pi_{\text{old}}$;
        \FOR{$k =1,\ldots,K$}
            %\STATE $\pi_{\theta_k} = \pi_{\theta_{\text{old}}}$;
            \STATE Simulate the current policy $\pi_{\theta_k}$ for $M$ steps and calculate the following two returns for every step $t=1,\ldots,M$: 
            \STATE $R_t = \sum_{j=t}^M \gamma^{j-t} r_j$;
            \STATE Estimate $A(s_t, a_t)$ using $R_t$ and $V_\phi(s_t)$;
            \STATE {\color{gray}\# Policy Improvement}
            \STATE $\theta_k^{(0)} = \theta_k$;
            \FOR{$i =0,\ldots,m-1$}
            \STATE $\theta_k^{(i+1)} \leftarrow \theta_k^{(i)} + \eta \left.\nabla_\theta\Psi(\theta,\theta_k)\right\vert_{\theta=\theta_k^{(i)}}$; $\quad$ (see Eq.~\ref{eq:grad0})
            %\STATE $g_{i} = \mathbb{E}_{s \sim \rho_{\pi_{k}}, a \sim \pi_{\theta_{old}}} \nabla_{\theta} \Bigl[\frac{\pi_{\theta}}{\pi_{\theta_{old}}} A^{\pi_{\theta_{old}}}(s, a) - \frac{1}{t_{k}} \mbox{KL} (\pi_{\theta}, \pi_{\theta_{old}}) \Bigr] \Bigm\lvert_{\theta = \theta{i}}$
            \ENDFOR
            \STATE $\theta_{k+1} = \theta_k^{(m)}$;
            \STATE {\color{gray}\# Policy Evaluation}
            \STATE Update $\phi$ by minimizing the $N$-batch loss function \\ $\quad L_{V_\phi} =\frac{1}{N} \sum_{t=1}^N\big[V_\phi(s_t) - R_t\big]^2$;
        \ENDFOR
        \vspace{0.4ex}
    \end{algorithmic}
\end{small}
\end{algorithm}
\end{minipage}%
\hfil % <===============================================================
\begin{minipage}[t]{6.777cm}%6cm <========================================== 
\begin{algorithm}[H]
\begin{small}
    \caption{Off-Policy MDPO}
    \label{alg:MDPO-OffPolicy}
    \begin{algorithmic}[1]
        \STATE {\bfseries Initialize} Replay buffer $\mathcal{D}=\emptyset$; $\;$ Policy networks $\pi_{\text{new}}$ and $\pi_{\text{old}}$; $\;$ and Value networks $V_\phi$ and $Q_\psi$; \\
        \FOR{$k =1,\ldots,K$}
            \STATE Take $a_k$ sampled from the current policy $\pi_{\theta_k}$, observe $r_k$ and $s_{k+1}$, and add $(s_k,a_k,r_k,s_{k+1})$ to $\mathcal{D}$;
            \STATE Sample a batch $\{(s_j, a_j, r_j, s_{j+1})\}_{j=1}^N$ from $\mathcal{D}$;
            \STATE {\color{gray}\# Policy update}
            \STATE Set the new policy $\theta_{k+1}$ by performing $m$ policy updates w.r.t.~the objective function $L_{\pi}(\theta, \theta_{k})$;
%            \FOR{$i =0,\ldots,m-1$}
%            \STATE Update $\theta$ w.r.t.~the objective $L(\theta, \theta_{k})$;
%            \ENDFOR
%            \STATE Set the new policy $\theta_{k+1}$ from the above loop;
            \STATE {\color{gray}\# Q and V updates}
            \STATE Update $\phi$ and $\psi$ w.r.t.~the following objective functions: \\ $L_{V_\phi} = \frac{1}{N}\sum_{j=1}^N\big(V_\phi(s_j)-Q_\psi(s_j,\pi_{\theta_{k+1}}(s_j))\big)^2$;
            \\ $L_{Q_\psi} \! = \! \frac{1}{N} \! \sum_{j=1}^N \!\! \big(r(s_j,a_j) + \gamma V_\phi(s_{j+1}) -  Q_\psi(s_j,a_j)\big)^2$;
        \ENDFOR
    \end{algorithmic}
\end{small}    
\end{algorithm}
\end{minipage}%
\end{comment}

%\vspace{0.5cm}
In comparison to TRPO, {\bf first,} on-policy MDPO does not explicitly enforce the trust-region constraint, but approximately satisfies it by performing multiple steps of SGD on the objective function of the optimization problem in the MD-style update rule~\eqref{MD Sample-based Theta}. We say ``{\em it approximately satisfies the constraint}'' because instead of fully solving~\eqref{MD Sample-based Theta}, it takes multiple steps in the direction of the gradient of its objective function. {\bf Second,} on-policy MDPO uses simple SGD instead of natural gradient, and thus, does not have to deal with the computational overhead of computing (or approximating) the inverse of the Fisher information matrix.\footnote{TRPO does not explicitly invert $F$, but instead, approximates the natural gradient update using conjugate gradient descent.} {\bf Third,} the direction of KL in on-policy MDPO, $\text{KL}(\pi,\pi_k)$, is consistent with that in the MD update rule in convex optimization and is different than that in TRPO, $\text{KL}(\pi_k,\pi)$. This does not cause any sampling problem for either algorithm, as both calculate the KL-term in closed-form (Gaussian policies). {\bf Fourth,}\label{point:tk} while TRPO uses heuristics to define the step-size and to reduce it in case the trust-region constraint is violated, on-policy MDPO uses a simple schedule, motivated by the theory of MD~\cite{beck2003mirror}, and sets $t_k\!=\!1\!-\!k/K$, where $K$ is the maximum number of iterations. This way it anneals the step-size $t_k$ from $1$ to $0$ over the iterations of the algorithm. 

%Finally, both TRPO and PPO deploy multiple heuristics in their implementations. For instance, the step size for the natural gradient step in TRPO is constantly halved until the KL constraint is met. In the case of MDPO, there is no such heuristic involved and we also provide a simple theoretically supported schedule for the KL coefficient in equation \ref{MD-TRPO}, which is a function of the current iteration $k$. \cite{beck2003mirror} show that $t_k$ is proportional to $\sqrt{k}$, where $k=1, 2, ..., T$. In order to realize this schedule, we anneal $\frac{1}{t_k}$ from 0 to 1 across the $T$ training steps. 

% \begin{equation}
% %\begin{array}{cc}
%     %& \displaystyle\max_{\theta} \ L_{\theta_{k}}(\theta) \\ \\
%     %& \mbox{s.t} \ \ \mbox{KL}(\pi_{\theta_{k}}, \pi_{\theta}) \leq \delta,
% %\end{array}
% \max_{\theta} \ L_{\theta_{k}}(\theta), \;\; \mbox{s.t. } \; \mbox{KL}(\pi_{\theta_{k}}, \pi_{\theta}) \leq \delta,
% \label{TRPO}
% \end{equation}

%where $L_{\theta_{k}}(\theta)$ is $\mathbb{E}_{s \sim \rho_{\theta_{k}}, a \sim \pi_{\theta}} [A^{\pi_{\theta_{k}}} (s, a)]$

%\manan{\textbf{Insert:} Comment on solving constrained vs unconstrained problem}

%Notice that TRPO argues for solving a constrained problem where there is a hard constraint on the trust region, realized through the target KL $\delta$. MDPO on the other hand, does not include a hard constraint, with the trust region requirement being maintained through the multi-step update. Furthermore, TRPO implements the above update through a natural policy gradient step, which requires inverting the Fisher information matrix $F$. Although $F$ can be approximated through optimization methods such as Conjugate Gradient Descent, there still exits a computational overload. In contrast, MDPO avoids this step as it uses simple SGD for its update. 

%\vspace{-0.025in}
{\bf Comparison with PPO:} At each iteration $k$, PPO performs multiple steps of SGD on the objective function of the following unconstrained optimization problem: 
%
%\vspace{-0.15in}
%\begin{small}
\begin{equation}
\begin{split}
\max_{\theta\in\Theta} \; \mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}&\Big[\min\Big\{\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)}A^{\theta_k}(s,a), \text{clip}\big(\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)},1-\epsilon,1+\epsilon\big)A^{\theta_k}(s,a)\Big\}\Big],
\label{eq:PPO-Opt}
\end{split}
\end{equation}
%\end{small}
%\vspace{-0.125in}
%
% \vspace{-0.275in}
% \begin{small}
% \begin{multline}
% \max_{\theta\in\Theta} \; \mathbb{E}_{\stackrel{s\sim\rho_{\theta_k}}{a\sim\pi_{\theta_k}}}\Big[\min\Big\{\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)}A^{\theta_k}(s,a), \\
% \text{clip}\big(\frac{\pi_\theta(a|s)}{\pi_{\theta_k}(a|s)},1-\epsilon,1+\epsilon\big)A^{\theta_k}(s,a)\Big\}\Big], %\nonumber
% \label{eq:PPO-Opt}
% \end{multline}
% \end{small}
% \vspace{-0.25in}
%
in which the hyper-parameter $\epsilon$ determines how the policy ratio, $\pi_\theta/\pi_{\theta_{k}}$, is clipped. It is easy to see that the gradient of the objective function in~\eqref{eq:PPO-Opt} is zero for the state-action pairs at which the policy ratio is clipped and is non-zero, otherwise. However, since the gradient is averaged over all the state-action pairs in the batch, the policy is updated even if its ratio is out of bound for some state-action pairs. This phenomenon, which has been reported in~\cite{wang2019truly} and~\cite{engstrom2019implementation}, shows that clipping in PPO does not prevent the policy ratios to go out of bound, but it only reduces its probability. This means that despite using clipping, PPO does not guarantee that the trust-region constraint is always satisfied. In fact, recent results, including those in~\cite{engstrom2019implementation} and our experiments in Section~\ref{subsection:on-policy-results}, show that most of the improved performance exhibited by PPO is due to code-level optimization techniques, such as learning rate annealing, observation and reward normalization, and in particular, the use of generalized advantage estimation (GAE)~\cite{schulman2015high}. %We delve deeper into this in Appendix A. %\mgh{This cannot be Appendix A, please fix.} 
Although both on-policy MDPO and PPO take multiple SGD steps on the objective function of unconstrained optimization problems~\eqref{MD Sample-based Theta} and~\eqref{eq:PPO-Opt}, respectively, the way they handle the trust-region constraint is completely different. 

Another interesting observation is that the adaptive and fixed KL algorithms (we refer to as KL-PPO here), proposed in the PPO paper~\cite{schulman2017proximal}, have policy update rules similar to on-policy MDPO. However, these algorithms have not been used much in practice, because it was shown in the same paper that they perform much worse than PPO. Despite the similarities, there are three main differences between the update rules of KL-PPO and on-policy MDPO. {\bf First,} KL-PPO uses mini-batches whereas MDPO uses the entire data for their multiple ($m$) gradient updates at each round. {\bf Second,} the scheduling scheme used for the $t_k$ parameter is quite different in KL-PPO and MDPO. In particular, KL-PPO either uses a fixed $t_k$ or defines an adaptive scheme that updates (increase/decrease) $t_k$ based on the KL divergence magnitude at that time step. On the other hand, on-policy MDPO uses an annealed schedule to update $t_k$, starting from $1$ and slowly bringing it down to near $0$. {\bf Third,} similar to TRPO, the direction of KL in KL-PPO, $\text{KL}(\pi_k,\pi)$, is different than that in on-policy MDPO, $\text{KL}(\pi,\pi_k)$. Since in our experiments, on-policy MDPO performs significantly better than PPO (see Section~\ref{subsection:on-policy-results}), we conjecture that either any or a combination of the above differences, especially the first two, is the reason for the inferior performance of KL-PPO, compared to PPO, as reported in~\cite{schulman2017proximal}.

%Another interesting observation is that the policy updates in the adaptive and fixed KL algorithms suggested in the PPO paper~\cite{schulman2017proximal} (referred here as KL-PPO) are quite similar to our on-policy MDPO algorithm. There are two main differences, \textbf{1)} there is no explicit mention of a multi-step SGD based update in KL-PPO. As discussed earlier in this section (right after Eq.~\ref{MD Sample-based Theta}), the single step SGD update of on-policy MDPO is equivalent to vanilla policy gradient, due to the fact that the gradient of the KL-term is zero. Also, \textbf{2)} as in the TRPO case, the direction of KL in on-policy MDPO, $\text{KL}(\pi,\pi_k)$, is consistent with the MD update and is different than that in KL-PPO, $\text{KL}(\pi_k,\pi)$. We conjecture that this is why~\citet{schulman2017proximal} reported that these algorithms do not work as well as PPO.  

%The authors propose different values for the KL penalty coefficient. In the one step case, this does not matter as the gradient is zero irrespective of the KL coefficient. However, they observe different results for different coefficient values. This contradicts the first statement. We suspect that this difference in results is due to the initial gradient step, which has a non zero KL gradient when the old and initial policies are not equal. This difference in gradient in the first step causes the eventual difference in results for different KL coefficients. This can be confirmed with a simple experiment and can be easily fixed by starting with the same old and new policies.

%Firstly, notice that the gradient of such an objective function for a particular state is zero when the probability ratio goes beyond the clipping range. However, note that when averaged across states, the batch gradient is non-zero and thus the policy is still updated, which in turn updates the ratio. Therefore, it can be easily realized that there is no constraint that stops the probability ratio to go out of bounds. The advantage provided by the clipping is that the gradient estimate is a "safer" estimate since some of its components are zero wherever the ratio is out of bound. This has been observed in other works as well \cite{wang2019truly}, \cite{engstrom2019implementation}. Therefore, although PPO and MDPO both solve an unconstrained problem, the way they handle the trust region requirement is completely different. Moreover, recent results suggest that most of the improved performance exhibited by PPO is due to code level optimizations present in its implementation. The algorithmic version of PPO has been shown to perform poorly in \cite{engstrom2019implementation}. This observation is reiterated in our experiments as well. \lior{what does it mean algorithmic version? We need to explain and use exact terms}

% \begin{remark}
% The adaptive and fixed KL algorithms suggested for the PPO algorithm in Schulman et al. \cite{schulman2017proximal} are exactly the one step SGD update in \ref{One step SGD}. The authors propose different values for the KL penalty coefficient. In the one step case, this does not matter as the gradient is zero irrespective of the KL coefficient. However, they observe different results for different coefficient values. This contradicts the first statement. We suspect that this difference in results is due to the initial gradient step, which has a non zero KL gradient when the old and initial policies are not equal. This difference in gradient in the first step causes the eventual difference in results for different KL coefficients. This can be confirmed with a simple experiment and can be easily fixed by starting with the same old and new policies.
% \end{remark}

% \begin{remark}
% In both TRPO and PPO, the KL is written as $\mbox{KL}(\pi_{k}, \pi)$ and not as $\mbox{KL}(\pi, \pi_{k})$. Clearly, since the KL is not symmetric, these two are not the same. By the Mirror Descent formulation, the latter is the correct way of defining the KL. Having said that, since TRPO solves each update using Natural Policy Gradient with a hard constraint on the KL term, the only place where this difference affects the results is in deciding the KL constraint (which might be negligible, as is supported by our experiments). %\lior{If the results indeed suggest similar performance, I'm not sure it is that interesting. We can omit it or shorten it. also, it shouldn't be a section, just a remark }
% \end{remark}



%\lior{This needs to be before the graphs. It could be here or in an experiments section. Depending on how everything is organized}


==> Sections/MDPO.tex <==
\vspace{-0.1in}
\section{Mirror Descent in RL}
\label{sec: MDPO}
\vspace{-0.05in}

% \manan{\textbf{Insert:} MDPO theory and basic introduction}

% \lior{I think we should have s short but thorough subsection here about the theory of MDPO. Think it should be before TRPO and SAC. Then, we should introduce briefly TRPO and SAC. Another format option is to introduce TRPO in section 3 (on-policy), and SAC 5 (off-policy). Another format option: Discuss here as you did - contrained vs. penalty, on-policy vs. off-policy}
% \manan{going with introducing TRPO, PPO and SAC as and when the MDPO versions are introduced, instead of having everything in the Prelims}
% \yon{There are two approaches discussed here, and it is important to differentiate between them: i) the uniform approach, in which you update all the state space (which closer to SAC), and ii) the TRPO approach, in which you update samples observed by acting with $\pi_k$.} 

The goal in RL is to find an optimal policy $\pi^*$. Two common notions of optimality, and as a result, two distinct ways to formulate RL as an optimization problem are as follows:
%
%\vspace{-0.175in}
%\begin{small}
\begin{subequations}
\label{eq:RL-Opt}
\[
\refstepcounter{equation}\latexlabel{eq:RL-Opt:partV}
\refstepcounter{equation}\latexlabel{eq:RL-Opt:partV0}
\text{\bf (a)} \;\;\; \pi^*(\cdot | s) \in \argmax_\pi \; V^\pi(s), \;\; \forall s\in\mathcal S, \qquad\qquad \text{\bf (b)} \;\;\; \pi^* \in \argmax_\pi \; \mathbb{E}_{s\sim\mu}\big[V^\pi(s)\big].
\tag{\ref{eq:RL-Opt}}
\]
\end{subequations}
%\end{small}
%\vspace{-0.175in}
%
% \vspace{-0.2in}
% \begin{small}
% \begin{align}
% \label{eq:RL-Opt-over-V}
% \text{\bf (a)} \quad \pi^*(\cdot | s) \in \argmax_\pi \; V^\pi(s), \;\; \forall s\in\mathcal S, \qquad\qquad \text{\bf (b)} \;\; \pi^* \in \argmax_\pi \; \mathbb{E}_{s\sim\mu}\big[V^\pi(s)\big].
% %\label{eq:RL-Opt-over-V0}
% \end{align}
% \end{small}
% \vspace{-0.225in}
%
In~\eqref{eq:RL-Opt:partV}, the value function is optimized over the entire state space $\mathcal S$. This formulation is mainly used in value function based RL algorithms. On the other hand, the formulation in~\eqref{eq:RL-Opt:partV0} is more common in policy optimization, where a scalar that is the value function at the initial state ($s\sim\mu$) is optimized.

Unlike the MD optimization problem, the objective function is not convex in $\pi$ in either of the above two RL optimization problems. %~\eqref{eq:RL-Opt-over-V} and~\eqref{eq:RL-Opt-over-V0}. 
Despite this issue,~\cite{geist2019theory} and~\cite{shani2019adaptive} have shown that we can still use the general MD update rule~\eqref{eq: md general update} and derive MD-style RL algorithms with the update rules
% The objective function is not convex in $\pi$ in either of these two optimization problems (unlike the MD optimization problem in Eq.~\ref{eq:MD-Opt}). Yet, it has been shown that we can still use the general MD update rule (Eq.~\ref{eq: md general update}) and derive RL algorithms with the following update rules
%
%\vspace{-0.175in}
%\begin{small}
\begin{align}
\label{MD Uniform}
&\pi_{k+1}(\cdot | s) \leftarrow \argmax_{\pi \in \Pi} \; \mathbb{E}_{a \sim \pi}\big[A^{\pi_{k}}(s, a)\big] - \frac{1}{t_{k}} \text{KL}(s;\pi,\pi_{k}), \quad\forall s\in\mathcal S, \\
&\pi_{k+1} \!\leftarrow \argmax_{\pi\in\Pi} \; \mathbb{E}_{s\sim\rho_{\pi_k}}\Big[\mathbb{E}_{a\sim\pi}\big[A^{\pi_{k}}(s, a)\big] \!-\! \frac{1}{t_{k}}\text{KL}(s;\pi,\pi_{k})\Big],
\label{MD Sample-based}        
\end{align}
%\end{small}
%\vspace{-0.175in}
%
for the optimization problems~\eqref{eq:RL-Opt:partV} and~\eqref{eq:RL-Opt:partV0}, respectively. Note that while in~\eqref{MD Uniform}, the policy is optimized uniformly over the state space $\mathcal S$, in~\eqref{MD Sample-based}, it is optimized over the measure $\rho_{\pi_{k}}$, i.e.,~the state frequency induced by the current policy $\pi_k$.


%Unlike the update rule~\eqref{MD Uniform}, in~\eqref{MD Sample-based}, the policy is optimized over the measure $\rho_{\pi_{k}}$, the state frequency induced by the current policy $\pi_k$. %In~\cite{shani2019adaptive}, the authors showed that replacing the `exact' update~\eqref{MD Sample-based} with its sample-based version results in an algorithm with similar performance to that of conservative policy iteration~\cite{kakade2002approximately}.  

%where we denote the above objective as $\Psi(\pi)$ \lior{A bit confusing choice of notation due to the already used $\psi$}.\yon{agree + delete this sentence once decide what to do with the notation}

In~\cite{shani2019adaptive}, the authors proved $\widetilde{\mathcal O}(1/\sqrt{K})$ convergence rate to the global optimum for these MD-style RL algorithms in the tabular case, where $K$ is the total number of iterations. They also showed that this rate can be improved to $\widetilde{\mathcal O}(1/K)$ in soft MDPs.\footnote{Note that in this case, the convergence is to the global optimum of the {\em soft} MDP (a biased solution).}
% It is promising that these rates are the same as those obtained in convex optimization for the MD algorithm~\cite{beck17FO}.
These results are important and promising, because they provide the same rates as those for MD in convex optimization~\cite{beck17FO}.

%Update rules~\eqref{MD Uniform} and~\eqref{MD Sample-based} form the basis for the two different versions of MDPO described in this work: (1) \emph{Off-policy MDPO} which uses samples from a replay buffer to estimate $A^\pi_k$ and then optimizes over the policy based as in \eqref{MD Uniform}. (2) \emph{On-policy MDPO} which performs updates using Monte-Carlo estimates of $A^{\pi_k}$ gathered by following the current policy, based on \eqref{MD Sample-based}.


% Recently, \cite{geist2019theory,shani2019adaptive} used the general MD update rule~\eqref{eq: md general update} to derive corresponding algorithms for RL by replacing $f(x)$ with the objective of RL. Two different objective functions were considered, (1) optimizing over $V^{\pi}(s)$ on the entire state space, and, (2) optimizing over the scalar function $\E_{s\sim \mu}[V^\pi(s)]$, i.e., optimizing over a scalar value function w.r.t. to the initial distribution $\mu$. 

% When the objective is to optimize $V^\pi(s)$ on the entire state space, applying the MD update rule results in the following update rule for all $s\in \mathcal{S}$
% \begin{equation}
%     \pi_{k+1}(\cdot | s) \leftarrow \displaystyle\arg\max_{\pi} \Bigl[\mathbb{E}_{a \sim \pi} A^{\pi_{k}}(s, a) - \frac{1}{t_{k}} \mbox{KL} (s; \pi, \pi_{k})\Bigr],
%     \label{MD Uniform}
% \end{equation}


% \begin{equation}
%     \pi_{k+1}(\cdot | s) \leftarrow \displaystyle\arg\max_{\pi} \mathcal{T}^{\pi} V^{\pi_{k}}(s) - \frac{1}{t_{k}} \mbox{KL} (s; \pi, \pi_{k}),
% \end{equation}
% where $\mathcal{T}^{\pi}$ is the linear Bellman operator. By subtracting the fixed term $\mathcal{T}^{\pi_k}V^{\pi_k}$, and using $\mathbb{E}_{a \sim \pi} A^{\pi_{k}}(s, a) = \mathcal{T}^{\pi} V^{\pi_{k}}(s) - \mathcal{T}^{\pi_k} V^{\pi_{k}}(s) $, we have
% \vspace{-0.3cm}


% Instead, applying MD for optimizing over the scalar function $\E_{s\sim \mu}[V^\pi(s)]$ results in the following update rule:
% % When working in the on-policy regime, i.e., when the states are can only be generated by following the current policy $\pi_k$, updating each state (uniform updates) is not possible. Therefore, similarly to \cite{shani2019adaptive}, we resort to sampling across states according to the current policy and the MD iterate can be written,
% \begin{equation}
%     \pi_{k+1} \leftarrow \displaystyle\arg\max_{\pi} \mathbb{E}_{s \sim \rho_{\mu,\pi_{k}}} \Bigl[\mathbb{E}_{a \sim \pi} A^{\pi_{k}}(s, a) - \frac{1}{t_{k}} \mbox{KL} (s; \pi, \pi_{k})\Bigr].
%     \label{MD Sample-based}.
% \end{equation}




==> Sections/RelatedWork.tex <==
%\vspace{-0.2cm}
\section{Related Work}
%\vspace{-0.2cm}
Recently, several works~\cite{neu2017unified,geist2019theory,shani2019adaptive} established theoretical convergence guarantees for the trust-region class of algorithms by drawing connections between  them and the mirror descent (MD) algorithm. Although the close relation between MD and policy optimization has been studied, to the best of our knowledge, there is only a single work that empirically studied the practical outcomes of this relation~\cite{mei2018exploration}. This work focuses on the off-policy case and proposes an algorithm, called Exploratory Conservative Policy Optimization (ECPO), that resembles our soft off-policy MDPO algorithm, except in the direction of the KL term. Although changing the direction of KL from mode seeking or \emph{reverse} (used by off-policy {\small MDPO}) to mean seeking or \emph{forward} has the extra overhead of estimating the normalization term (see Eqs.~\ref{eq:off-policy-MDPO-update1} and~\ref{eq:off-policy-MDPO-update2}),~\citet{mei2018exploration} argue that it results in better performance. They show this by comparing {\small ECPO} with a number of algorithms, including one that is close to our off-policy {\small MDPO} and they refer to as Policy Mirror Descent (PMD). They specifically report poor performance for {\small PMD} in their experiments. Although we did not use their code-base and their exact configuration, we did not observe such poor performance for our off-policy {\small MDPO} algorithm (that uses the mode seeking KL direction). In fact, our experimental results in Section~\ref{subsection:off-policy-results} show that off-policy {\small MDPO} performs better than or on-par with {\small SAC} in six commonly used MuJoCo domains. More experiments and further investigation are definitely required to explain this discrepancy and identify the settings suitable for each algorithm.
% Policy optimization methods progress by `slowly' changing the policy towards an improved one. It has been shown that this slow change results in theoretically sound algorithms, such as Conservative Policy Iteration (CPI)~\cite{kakade2002approximately}. Motivated by CPI, powerfull algorithms such as TRPO~\cite{schulman2015trust} and PPO~\cite{schulman2017proximal} have been developed that enforced consecutive policies to remain `close' to one another by directly encoding this requirement into the optimization problem. This class of RL algorithms are referred to as trust region methods.% 
% \lior{HI, I think the first paragraph was just repeating things we've already said, what do you think? We need everything including references be no more than 10 pages}
%builds upon the connection between policy optimization and MD and propose an off-policy actor critic style algorithm which closely resembles soft off-policy MDPO. The difference is in the order of the KL divergence used to optimize the parameterized policy toward the closed form solution (see equation \ref{eq:off-policy-MDPO-update2}). They argue for a reversed order of KL divergence and in fact claim that using the order used in \ref{eq:off-policy-MDPO-update2} leads to very poor performance. However, we clearly show that such is not the case. Further investigation is required to explain this discrepancy in results. 
